CROP: Certifying Robust Policies for Reinforcement Learning through Functional Smoothing

As reinforcement learning (RL) has achieved great success and been even adopted in safety-critical domains such as autonomous vehicles, a range of empirical studies have been conducted to improve its robustness against adversarial attacks. However, how to certify its robustness with theoretical guarantees still remains challenging. In this paper, we present the first unified framework CROP (Certifying Robust Policies for RL) to provide robustness certification on both action and reward levels. In particular, we propose two robustness certification criteria: robustness of per-state actions and lower bound of cumulative rewards. We then develop a local smoothing algorithm for policies derived from Q-functions to guarantee the robustness of actions taken along the trajectory; we also develop a global smoothing algorithm for certifying the lower bound of a finite-horizon cumulative reward, as well as a novel local smoothing algorithm to perform adaptive search in order to obtain tighter reward certification. Empirically, we apply CROP to evaluate several existing empirically robust RL algorithms, including adversarial training and different robust regularization, in four environments (two representative Atari games, Highway, and CartPole). Furthermore, by evaluating these algorithms against adversarial attacks, we demonstrate that our certification are often tight. All experiment results are available at website https://crop-leaderboard.github.io.

==> [ICLR2022] robust-RL-CROP/archive/smooth_policy.tex <==
\subsection{Randomized Smoothing on Policies}

% See Section 3.3, Theorem 5, and Theorem 6 in~\cite{zhang2021robust}.

\begin{definition}[percentile smoothing~\cite{chiang2020detection}]
\label{def:median-smooth}
Given $f:\bb R^d\rightarrow \bb R$ and $G\sim\cal N(0,\sigma^2I)$, the percentile smoothing of $f$ is defined as:
\begin{align*}
\tilde f_{p}(x)&=\sup \{y \in \mathbb{R} \mid \mathbb{P}[f(x+G) \leq y] \leq p\}
\end{align*}
\end{definition}

For each action dimension $\mu(a^i|s)$, we apply percentile smoothing in~\Cref{def:median-smooth} to get $\tilde\mu(a^i|s)$.

\begin{lemma}[\cite{chiang2020detection}]
\label{lem:median-smooth}
A percentile-smoothed function $h_p$ with adversarial perturbation $\delta$ can be bounded as
\begin{align*}
    {h}_{\underline p}(x) \leq h_{p}(x+\delta) \leq {h}_{\bar{p}}(x) \quad \forall\|\delta\|_{2}<\epsilon,
\end{align*}
where $\underline{p}:=\Phi\left(\Phi^{-1}(p)-\frac{\epsilon}{\sigma}\right)$ and $\bar{p}:=\Phi\left(\Phi^{-1}(p)+\frac{\epsilon}{\sigma}\right)$, with $\Phi$ being the standard Gaussian CDF.
\end{lemma}

According to Lemma~\ref{lem:median-smooth}, the output action of the smoothed policy network will be bounded under attack.

\begin{lemma}[\cite{zhang2021robust}]
\label{lem:v-bound-dtv}
Given a policy $\pi$ and its value function $V^\pi(s)$. Denote the value function under the state perturbation of $\nu_\eps$ as $V_\eps^\pi(s)$. For all $s\in \cal S$, we have
\begin{align*}
    V^{\pi}(s)-{V}_{\eps}^\pi(s) \leq \alpha \max _{s \in \mathcal{S}}  \dtv(\mu(\cdot \mid s), \mu(\cdot \mid s+\nu_\eps(s))),
\end{align*}
where $\dtv(\mu(\cdot| s), \mu(\cdot|s+\nu_\eps(s)))$ is the total variation distance between $\mu(\cdot|s)$ and $\mu(\cdot|s+\nu_\eps(s))$, 
and $\alpha\triangleq 2\left[1+\frac{\gamma}{(1-\gamma)^{2}}\right] \max _{\left(s, a, s^{\prime}\right) \in \mathcal{S} \times \mathcal{A} \times \mathcal{S}}\left|R\left(s, a, s^{\prime}\right)\right|$ is a constant that does not depend on $\pi$.
\end{lemma}

\begin{theorem}
\label{thm:dtv-mu}
\begin{align*}
    \dtv(\mu(\cdot \mid s), \mu(\cdot \mid s+\nu_\eps(s)))\le\sum\left(\tilde\mu_{\bar p}(a^i|s)-\tilde\mu_{\underline p}(a^i|s) \right)
\end{align*}
\end{theorem}
\begin{proof}
    Immediate from Lemma~\ref{lem:median-smooth}.
\end{proof}
Combining Lemma~\ref{lem:v-bound-dtv} and~\Cref{thm:dtv-mu}, we conclude that the performance gap of the smoothed policy $\tilde \mu$ under clean and perturbed test environment will be bounded.

\textbf{next step}: check whether there is a tighter bound than Lemma~\ref{lem:v-bound-dtv}.

==> [ICLR2022] robust-RL-CROP/archive/thm-global-smoothing.tex <==
        \begin{theorem}
            Let $\pi'=\pi(s+\Delta)$ where $\Delta \sim \gN(0,\sigma^2I_S)$, $J(\pi')$ is 
            
            When $\norm{\delta_i}_2\leq \eps$ for all $i$, 
            $\wtilde F(\delta_1^m, \delta_2^m,\ldots, \delta_H^m)$ is lower bounded by
            % $\wtilde F(0,0,\ldots,0)-(R_{\max}-R_{\min})\sqrt{\frac{\ln(1/\alpha)}{2m}} - L\eps\sqrt{H}$
            $\wtilde F(0,0,\ldots,0) - L\eps\sqrt{H}$.
            % with $m$ sampled macro-states and confidence parameter $\alpha$. 
            % $R_{\max}$ and $R_{\min}$ are the maximum and minimum cumulative reward of the game known a priori, and  
            $L$ is the \lip constant in~\Cref{lem:global-lip}.
        \end{theorem}

==> [ICLR2022] robust-RL-CROP/archive/thm-proof-radius.tex <==
\iffalse
\begin{proof}
We first present the bound for the smoothed value function $\wtilde V^\pi$. For each $s \in \cal S$, given the local \lip continuity of the smoothed $\wtilde Q^\pi$ (\Cref{lem:lipschitz}), we have
    \begin{align*}
        \wtilde V_\eps^\pi(s)-\wtilde V^\pi(s)
&=      \wtilde V^\pi (s + \nu_\eps(s)) - \wtilde V^\pi (s)\\
&=        \max_{a_1}\wtilde Q^\pi(s+\nu_\eps(s),a_1)-\max_{a_2}\wtilde Q^\pi(s,a_2)\\
&\geq     \wtilde Q^\pi(s+\nu_\eps(s),a)-\wtilde Q^\pi(s,a)\qquad\qquad \textit{ where } a=\argmax_{a_2}\wtilde Q^\pi(s,a_2)\\
&\geq     -L_s \cdot \eps
\end{align*}
The bound on the other side can be similarly derived.

Next, we compute the certified radius at state $s$. 
Let $\hat s$ be the adversarial state observation satisfying the constraint $\norm{\hat s-s}\leq \eps$. 
Leveraging the property that $\eta_s_a$ is $1$-\lip in $\cal N(s)$ given in~\Cref{lem:1-lip}, we have
% compute the certified radius as follows.
% For any $\delta$ with $\norm{\delta}_2\leq \eps$,
\begin{align}
    \label{eq:r-1}
    & \left(\textit{Due to \lip continuity}\right) 
    & \eta_{\hat s}^{(a_1)}(s) - \eta_{\hat s}^{(a_1)}(\hat s) \leq \eps \\
    \label{eq:r-2}
    & \left(\textit{Property of adversarial example}\right) 
    & \eta_{\hat s}^{(a_1)}(\hat s) \leq \eta_{\hat s}^{(a_2)}(\hat s)\\
    % \label{eq:r-3}
    % & \left((\textit{\ref{eq:r-1}) + (\ref{eq:r-2})}\right) 
    % & \eta_{a_1}(s) \leq \eta_{a_2} (\hat s) + \norm{\delta}_2\\
    \label{eq:r-4}
    & \left(\textit{Due to \lip continuity}\right)
    & \eta_{\hat s}^{(a_2)}(\hat s) - \eta_{\hat s}^{(a_2)}(s) \leq \eps\\
    \label{eq:r-5}
    & \left(\textit{(\ref{eq:r-1}) + (\ref{eq:r-2}) + (\ref{eq:r-4})}\right) 
    & \eta_{\hat s}^{(a_1)}(s) - \eta_{\hat s}^{(a_2)}(s) \leq 2\eps.
\end{align}
Thus, to allow for the existence of an adversarial example within perturbation budget $\eps$, the following condition needs to be satisfied:
\begin{align}
    \label{eq:r-cond}
    \eps 
    &\geq \min_{\substack{s'\\\st\norm{s'-s}_2\leq \eps}} \frac{1}{2}\left( \eta_{\hat s}^{(a_1)}(s) - \eta_{\hat s}^{(a_2)}(s) \right).
\end{align}
The certified radius $R(s)$ at state $s$ is thus the smallest $\eps$ for Ineq. (\ref{eq:r-cond}) to hold.


Thus, the magnitude of the perturbation applied to state $s$ shall at least 

in order to mislead the action given by $\tilde \pi$, the perturbation magnitude shall at least be 
% $\frac{1}{2}\left(\eta_{a_1}(s) - \eta_{a_2} (s)\right)$, \ie,
% which implies that the induced action will not change within
\begin{align*}
        R(s) &= \frac{1}{2}\left(\eta_{a_1}(s) - \eta_{a_2} (s)\right) \\
             &=
        \frac{\sigma}{2}\left(
    \Phi^{-1}\left(\frac{\wtilde Q(s,a_1)-V_{\min}}{V_{\max}-V_{\min}}\right)-
    \Phi^{-1}\left(\frac{\wtilde Q(s,a_2)-V_{\min}}{V_{\max}-V_{\min}}\right)
    \right).
\end{align*}
\end{proof}
\fi


==> [ICLR2022] robust-RL-CROP/archive/thm-q-bound.tex <==
\begin{theorem}
\label{thm:radius}
% Let $Q^\pi$ be the action value function given by the trained $Q$ network with policy $\pi$.
% Assume $\wtilde Q^\pi$ is the smoothed $Q^\pi$ given by~\Cref{eq:smooth-q}, and $\tilde\pi$ is the policy induced by the smoothed action value function $\wtilde Q^\pi$ following~\Cref{alg:smooth-q}.
Let $Q^\pi: \cal S \times \cal A\rightarrow \bb R$ be a trained value network, 
$\wtilde Q^\pi$ be the smoothed action-value function given in~\Cref{eq:smooth-q} and $\wtilde V^\pi$ be the smoothed value function given in~\Cref{eq:smooth-v}.
We further define $\wtilde V_\eps^\pi(s) := \wtilde V^\pi (s + \nu_\eps(s)) $ as the test-time value function given a perturbation $\nu_\eps(s):\cal S\rightarrow \cal S$ within magnitude $\eps$ on the input state observation $s$.
Then for any $s\in \cal S$,
\begin{align*}
    |\wtilde V_\eps^\pi(s)-\wtilde V^\pi(s)|\in [-L_s\eps, L_s\eps].
\end{align*}
Further, we can certify a radius $R$ at state $s$, such that when the perturbation scale is smaller than $R(s)$, the induced action at state $s$ will not change. The radius $R(s)$ is defined below
\begin{align*}
    R(s)
    &:= \frac{1}{2}\left( \eta_{a_1}(s) - \eta_{a_2}(s) \right).
\end{align*}
% \begin{align*}
%         R(s) := \frac{\sigma}{2}\left(
%     \Phi^{-1}\left(\frac{\wtilde Q(s,a_1)-V_{\min}}{V_{\max}-V_{\min}}\right)-
%     \Phi^{-1}\left(\frac{\wtilde Q(s,a_2)-V_{\min}}{V_{\max}-V_{\min}}\right)
%     \right),
% \end{align*}
where $a_1$ is the action of the highest smoothed $\wtilde Q$ value, while $a_2$ is the runner-up action.
\end{theorem}


==> [ICLR2022] robust-RL-CROP/certify-algs.tex <==
{


\section{Na\"ive Certification Approaches for Actual Reward Bounds}

    This section contains the certification approaches considering the actual reward bounds.
    These algorithms are suitable for both value-based neural networks and policy-based neural networks.
    
    \subsection{Notations}
        Given a \emph{deterministic} policy $\pi$, we define the \emph{actual reward} by
        \begin{align}
            \bar Q^\pi(s,a) & := \E\left[ \sum_{t=0}^\infty \gamma^t r_t \Big| s_0 = s, a_0=a, \pi\right], \\
            \bar V^\pi(s) & := \E\left[ \sum_{t=0}^\infty \gamma^t r_t \Big| s_0 = s, \pi\right], \\
            J(\pi) & := \E\left[\sum_{t=0}^\infty \gamma^t r_t \Big| s_0 \sim d_0, \pi\right].
        \end{align}

    \subsection{Certifying Globally Randomized Policy: Global Smoothing}
    
        For the given deterministic policy $\pi$, we construct a randomized policy $\pi'$.
        At each step, this randomized policy $\pi'$ adds one-time perturbation $\delta \sim \gN(0,\sigma^2I)$ to the observed state $s$, and make decision according to $\pi(s + \delta)$.
        Note that that $\pi'$ is different from the smoothed policy defined in main text.
        Because at each step, we just add one noise and make the decision according to this single noised state instead of adding multiple noises and make the decision according to the majority vote.
        
        We assume that each epoch has at most $H$ time steps, each state has $s$ dimensions.
        Then, we define a function $F: \sR^{H \times S} \to \sR$ such that
        \begin{align}
            F(\delta_1,\delta_2,\dots,\delta_H) = \E
            \left[
                \sum_{t=0}^H \gamma_t r_t \Big| s_0 \sim d_0, s_i = \pi(s_{i-1}, \delta_i)
            \right],
        \end{align}
        where $\delta_i \in \sR^S$ is the perturbation added to each step.
        Furthermore, we define smoothed $F$ by $\tilde F: \sR^{H\times S} \to \sR$:
        \begin{align}
            & \tilde F(s_1,s_2,\dots,s_H) \nonumber \\
            = & 
            \underset{\substack{\delta_i \sim \gN(0,\sigma^2I_S),\\ 1\le i\le H}}{\E} F(s_1+\delta_1,s_2+\delta_2,\dots,s_H+\delta_H).
        \end{align}
        
        According to the definition, 
        \begin{align}
            J(\pi') = \underset{\substack{\delta_i \sim \gN(0,\sigma^2I_S),\\ 1\le i\le H}}{\E} F(\delta_1,\delta_2,\dots,\delta_H) = \tilde F(0,\dots,0).
        \end{align}
        We let $(\delta_1',\delta_2',\cdots,\delta_H')$ be the state perturbation added to each step.
        Then, the resulting actual reward received under the perturbation by policy $\pi'$ is exactly
        \begin{align}
            \tilde F(\delta_1',\delta_2',\cdots,\delta_H').
        \end{align}
        As a result, we can sample to estimate $\tilde F(0,\cdots,0) = J(\pi')$~(using Hoeffding's Inequality to get a high confidence bound).
        Then, we can leverage the smoothness property of $\tilde F$~\cite{salman2019provably,chiang2020detection} to obtain a lower bound of $\tilde F(\delta_1', \delta_2', \dots,\delta_H')$, which is a valid certification of the actual reward for the randomized policy $\pi'$.

        \begin{remark}
            Regardless of the input dimension, the certification of the smoothed function has a similar magnitude as long as the noise variance $\sigma$ is the same.
            For example, when $\sigma = 1.0$, the non-trivial robustness certification usually requires the perturbation be bounded by $\ell_2$ under $1.0$---$2.0$.
            Thus, if the input dimension is too high, the permitted noise per component is too small~(scales down in $1/\sqrt{d}$ rate).
            
            For the classification, the input dimension is exactly the image size.
            However, for reinforcement learning, this global smoothing strategy produces an input dimension $H\times S$.
            If the state is an image, it is about $H$ times larger than the dimension of the classification task.
            Therefore, the certified robustness would be coarse.
            
            A potential direction is to reduce the dimension of state observation.
            We may train the policy in low-dimensional space, and certify the projection from high dimension to low dimension is robust. 
            Then the whole pipeline may have nontrivial certified robustness.
            The idea would be in spirit similar to low-rank approximation for certified robustness~\cite{awasthi2020adversarial}.
        \end{remark}
        
        \begin{remark}
            To yield a good randomized policy $\pi'$, the original policy should be trained to still have good performance under Gaussian corrupted state observations.
            In other words, it is necessary to train the policy using Gaussian augmentation on the state observation.
        \end{remark}
    
        % \fan{pseudo code see~\Cref{alg:global-rand}}
        % \input{pseudo-code/global-certify}
    
    \subsection{Certifying Stepwise Smoothed Policy: Adaptive Search}
        
        
        \paragraph{Prerequisite.}
        Either the test environment supports state saving or backtracking, either the state transition is deterministic.
        
        For the given deterministic policy $\pi$, suppose the policy uses per-step smoothing, which corresponding to using $\tilde Q$ for value network or pure smoothing for policy network.
        Then, at each step $i$, we can easily derive a certified robust radius $r_i$, such that the perdicted action $a_i$ does not change as long as the state observation is perturbed within $\ell_2$ radius $r_i$.
        Moreover, by comparing the smoothed confidence for each action, or the smoothed $\tilde Q$ for each action, we can know that if the perturbation goes beyond $r_i$, what action(s) it might take.
        Formally,
        we would have $r_{i,a'}$ for each action $a'$ different from the benign action, such that within $r_{i,a'}$ at least the policy would not choose $a'$.
    
        We assume that the initial state is fixed to $s_0$.
        
        First, we run the policy $\pi$ without any state perturbation starting from $s_0$, until it finishes an epoch with $H$ time steps.
        We record the actual reward as $J(\pi)$ and the per-step certified radius as $r_i$ where $1\le i\le H$.
        Now, we know the actual reward lower bound is $J(\pi)$ as long as the perturbation per step is within $\min_{1\le i\le H} r_i$.
        
        For notation simplicity, we let $i_0 = \argmin_{1\le i\le H} r_i$.
        Thus, $\min_{1\le i\le H} r_i = r_{i_0}$.
        
        We start to enlarge the radius from $r_{i_0}$.
        We spot the runner-up action at step $i_0$, which is denoted as $a^{adv}_{i_0}$.
        We then figure out $r^{new}$, such that under perturbation within $r^{new}$, for all steps other than $i_0$ it is still robust, and only on step $i_0$, we may choose either $a_{i_0}$ or $a^{adv}_{i_0}$.
        Apparently, we have $r^{new} > r_{i_0}$.
        We start to explore the trajectory $s_0,a_0,s_1,a_0,\cdots,s_{i_0},a_{i_0}^{adv}$.
        For the steps $i$'s following $i_0$, we explore all possible actions $a$ with certified radius $r_{i,a} \le r_{i_0}$.
        We record the lowest actual reward we get as $J'$.
        Then, the actual reward lower bound is $J'$ as long as the perturbation is within $r^{new}$.
        Here, $r^{new}$ is the minimum certified radius that is  larger than $\min_{1\le i\le H} r_i$ among all steps we encountered during the process.
        
        We repeat the process to enlarge the radius from $r^{new}$.
        The process can be viewed as generating new branches from a trajectory tree.
        The algorithm can be terminated at any time.
        As a possible optimization, notice the decay factor $\gamma$---we may do early stopping with bounded loss to accelerate.
        
        \begin{remark}
            At a high level, the algorithm is based on search.
            It goes through all possible trajectories to find the actual reward lower bound.
            The per-step smoothing provides the guarantee that we can determine all possible trajectories given the perturbation budget, which otherwise impossible.
        \end{remark}
        
        \begin{remark}
            In the supervised learning setting, for most samples, the certified radii are large.
            Only for a few samples, the certified radii are small.
            Simiarly, I conjecture that in the reinforcement learning case, there are just few steps with small certified radii.
            Thus, as long as we branch and search all these few steps, we can significantly enlarge the certified radius.
        \end{remark}
        
        \begin{remark}
            The existence of this algorithm also implies that, to certify the actual reward lower bound for a deterministic policy~(instead of expectation as before), maybe it is inevitable to examine every possible trajectory,
            since we do not know what would happen on the unexplored trajectory.
            It is essentially because we do not have the smoothness guarantee of $Q^*$, which is solely depended on the internal properties of the game and the reward. 
        \end{remark}
        
        % \fan{pseudo code see~\Cref{alg:adaptive-search}}
        % \input{pseudo-code/adaptive-search}
    
}

==> [ICLR2022] robust-RL-CROP/fig_desc/fig_Breakout_lore.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}


\begin{figure}



\newlength{\utilheightbreakout}
\settoheight{\utilheightbreakout}{\includegraphics[width=.3\linewidth]{figures/Breakout_adasearch_sigma-0.005.pdf}}%


\newlength{\legendheightbreakout}
\setlength{\legendheightbreakout}{0.25\utilheightbreakout}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightbreakout][c]{\small #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightbreakout]{figures/legend_Breakout.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{$\sigma=0.005$}}
        & \makecell{\small{$\sigma=0.01$}}
        & \makecell{\small{$\sigma=0.05$}}
        \vspace{-2pt}\\
\rowname{\makecell{(Local) $\uj$}}&
\includegraphics[height=\utilheightbreakout]{figures/Breakout_adasearch_sigma-0.005.pdf}&
\includegraphics[height=\utilheightbreakout]{figures/Breakout_adasearch_sigma-0.01.pdf}&
\includegraphics[height=\utilheightbreakout]{figures/Breakout_adasearch_sigma-0.05.pdf}
\\[-0.1ex]
        & \makecell{\small{attack epsilon $\eps$}}
        & \makecell{\small{attack epsilon $\eps$}}
        & \makecell{\small{attack epsilon $\eps$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \mo{\textbf{Robustness certification for cumulative reward lower bound $\uj$  on \textit{Breakout}}. We evaluate the trajectory length $H=200$. Each column corresponds to one smoothing parameter $\sigma$. Different lines represent the certified reward bounds of different RL methods.}
}%
\label{fig:breakout-lore}
\end{figure}



==> [ICLR2022] robust-RL-CROP/fig_desc/fig_cartpole.tex <==
{
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}


\newlength{\cputilheighta}
\settoheight{\cputilheighta}{\includegraphics[width=.160\linewidth]{figures/Freeway_stepwise_sigma-0.001.pdf}}%

\newlength{\cpwrapheighta}
\settoheight{\cpwrapheighta}{\includegraphics[width=.400\textwidth]{figures/CartPole_loact_clean.pdf}}%

\newlength{\cplegendheight}
\setlength{\cplegendheight}{0.3\cputilheighta}%


\newcommand{\cprowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\cputilheighta][c]{\tiny #1}}}


\newlength{\cputilheightc}
\settoheight{\cputilheightc}{\includegraphics[width=.160\linewidth]{figures/Freeway_global_mean_sigma-0.001.pdf}}%

\newlength{\cputilheightd}
\settoheight{\cputilheightd}{\includegraphics[width=.165\linewidth]{figures/Freeway_global_median_sigma-0.001.pdf}}%


\newlength{\cputilheightaa}
\settoheight{\cputilheightaa}{\includegraphics[width=.162\linewidth]{figures/Freeway_adasearch_sigma-0.05.pdf}}%

\newlength{\cputilheightcp}
\settoheight{\cputilheightcp}{\includegraphics[width=.160\linewidth]{figures/CartPole_global_mean_sigma-0.001_cmp.pdf}}%

\newlength{\cputilheightdp}
\settoheight{\cputilheightdp}{\includegraphics[width=.165\linewidth]{figures/CartPole_global_median_sigma-0.001_cmp.pdf}}%


\newlength{\cputilheightaap}
\settoheight{\cputilheightaap}{\includegraphics[width=.162\linewidth]{figures/CartPole_adasearch_sigma-0.05_cmp.pdf}}%


% \newlength{\cputilheight}
% \settoheight{\cputilheight}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: low degree.pdf}}%

% \newlength{\attackheightb}
% \settoheight{\attackheightb}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: high degree.pdf}}%

\newlength{\cplegendheightb}
\setlength{\cplegendheightb}{0.3\cputilheightc}%


\newcommand{\cprownamec}[1]% #1 = text
{\rotatebox{90}{\makebox[\cputilheightc][c]{\tiny #1}}}

\newcommand{\cprownamed}[1]% #1 = text
{\rotatebox{90}{\makebox[\cputilheightd][c]{\tiny #1}}}



\centering



{
\renewcommand{\tabcolsep}{10pt}

\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\cplegendheight]{figures/Cartpole_legend.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\cprowname{\makecell{CartPole\\Radius $r$}}&
\includegraphics[height=\cputilheighta]{figures/CartPole_stepwise_sigma-0.001.pdf}&
\includegraphics[height=\cputilheighta]{figures/CartPole_stepwise_sigma-0.005.pdf}&
\includegraphics[height=\cputilheighta]{figures/CartPole_stepwise_sigma-0.01.pdf}&
\includegraphics[height=\cputilheighta]{figures/CartPole_stepwise_sigma-0.03.pdf}&
\includegraphics[height=\cputilheighta]{figures/CartPole_stepwise_sigma-0.05.pdf}&
\includegraphics[height=\cputilheighta]{figures/CartPole_stepwise_sigma-0.1.pdf}\\[-1.2ex]
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
\end{tabular}
\caption{\small Robustness certification for \textit{per-state action} in terms of certified radius $r$ at all time steps.
% We consider six methods: StdTrain, GaussAug, AdvTrain, RegPGD, RegCVX, and RadialRL, with the last three being SOTA. 
The shaded area represents the standard deviation.
% RadialRL is the most certifiably robust method on Freeway, while RegCVX is the most robust on CartPole.
}%
\label{fig:cartpole-statewise}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}


\begin{subtable}[]{\linewidth}
\centering
\includegraphics[height=\cpwrapheighta]{figures/Cartpole_loact_clean.pdf}
\vspace{-1mm}
\caption{\small Benign performance of  locally smoothed policy $\tpi$ under different  smoothing variance $\sigma$.}\label{fig:cartpole-statewise-clean}
\end{subtable}

\vspace{1em}

\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\cplegendheightb]{figures/CartPole_legend_marker.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{3mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\tiny{$\sigma=0.001$}}
        & \makecell{\tiny{$\sigma=0.005$}}
        & \makecell{\tiny{$\sigma=0.01$}}
        & \makecell{\tiny{$\sigma=0.03$}}
        & \makecell{\tiny{$\sigma=0.05$}}
        & \makecell{\tiny{$\sigma=0.1$}}
        \vspace{-1.7pt}\\
\cprownamec{\makecell{(Global) $\uje$}}&
\includegraphics[height=\cputilheightcp]{figures/CartPole_global_mean_sigma-0.001_cmp.pdf}&
\includegraphics[height=\cputilheightcp]{figures/CartPole_global_mean_sigma-0.005_cmp.pdf}&
\includegraphics[height=\cputilheightcp]{figures/CartPole_global_mean_sigma-0.01_cmp.pdf}&
\includegraphics[height=\cputilheightcp]{figures/CartPole_global_mean_sigma-0.03_cmp.pdf}&
\includegraphics[height=\cputilheightcp]{figures/CartPole_global_mean_sigma-0.05_cmp.pdf}&
\includegraphics[height=\cputilheightcp]{figures/CartPole_global_mean_sigma-0.1_cmp.pdf}\\[-1.2ex]
\cprownamed{\makecell{(Global) $\ujp$}}&
\includegraphics[height=\cputilheightdp]{figures/CartPole_global_median_sigma-0.001_cmp.pdf}&
\includegraphics[height=\cputilheightdp]{figures/CartPole_global_median_sigma-0.005_cmp.pdf}&
\includegraphics[height=\cputilheightdp]{figures/CartPole_global_median_sigma-0.01_cmp.pdf}&
\includegraphics[height=\cputilheightdp]{figures/CartPole_global_median_sigma-0.03_cmp.pdf}&
\includegraphics[height=\cputilheightdp]{figures/CartPole_global_median_sigma-0.05_cmp.pdf}&
\includegraphics[height=\cputilheightdp]{figures/CartPole_global_median_sigma-0.1_cmp.pdf}\\[-1.2ex]
\cprownamed{\makecell{(Local) $\uj$}}&
\includegraphics[height=\cputilheightaap]{figures/CartPole_adasearch_sigma-0.001_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/CartPole_adasearch_sigma-0.005_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/CartPole_adasearch_sigma-0.01_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/CartPole_adasearch_sigma-0.03_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/CartPole_adasearch_sigma-0.05_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/CartPole_adasearch_sigma-0.1_cmp.pdf}\\[-1.2ex]
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
\end{tabular}
}
\caption{\small Robustness certification as cumulative reward, including \textit{expectation bound} $\uje$, \textit{percentile bound} $\ujp$ ($p=50\%$), and \textit{absolute lower bound} $\uj$. 
% Each column corresponds to one smoothing variance. 
Solid lines represent the certified reward bounds of different methods, and dashed lines show the empirical performance under PGD attacks.}\label{tab:cartpole-bounds}
\end{subtable}
}

\caption{\small \textbf{Robustness certification on CartPole} in terms of (a-b): \textit{robustness of per-state action} and (c): \textit{lower bound of cumulative rewards}.
In (a) and (c), each column corresponds to one smoothing variance. 
% , including as cumulative reward, including \textit{expectation bound} $\uje$, \textit{percentile bound} $\ujp$ ($p=50\%$), and \textit{absolute lower bound} $\uj$  on (a) Freeway and (b) Pong. Each column corresponds to one smoothing variance. Solid lines represent the certified reward bounds of different methods, and dashed lines show the empirical performance under PGD attacks.
}\label{tab:cartpole-figs}
\end{figure}

}


==> [ICLR2022] robust-RL-CROP/fig_desc/fig_certified_ratio.tex <==
\begin{figure}
\newlength{\utilheightb}
\settoheight{\utilheightb}{\includegraphics[width=.165\linewidth]{figures/Freeway_stepwise_ratio_sigma-0.001.pdf}}%

\newlength{\legendheightratio}
\setlength{\legendheightratio}{0.3\utilheightb}%

\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightb][c]{\tiny #1}}}

\centering


{
\renewcommand{\tabcolsep}{10pt}

\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightratio]{figures/legend_simp.pdf}
\end{tabular}
\end{subtable}



\begin{subtable}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\rowname{\makecell{Freeway\\ratio \%}}&
\includegraphics[height=\utilheightb]{figures/Freeway_stepwise_ratio_sigma-0.005.pdf}&
\includegraphics[height=\utilheightb]{figures/Freeway_stepwise_ratio_sigma-0.05.pdf}&
\includegraphics[height=\utilheightb]{figures/Freeway_stepwise_ratio_sigma-0.1.pdf}&
\includegraphics[height=\utilheightb]{figures/Freeway_stepwise_ratio_sigma-0.5.pdf}&
\includegraphics[height=\utilheightb]{figures/Freeway_stepwise_ratio_sigma-0.75.pdf}&
\includegraphics[height=\utilheightb]{figures/Freeway_stepwise_ratio_sigma-1.0.pdf}\\[-1.2ex]
\rowname{\makecell{Pong\\ratio \%}}&
\includegraphics[height=\utilheightb]{figures/Pong_stepwise_ratio_sigma-0.001.pdf}&
\includegraphics[height=\utilheightb]{figures/Pong_stepwise_ratio_sigma-0.005.pdf}&
\includegraphics[height=\utilheightb]{figures/Pong_stepwise_ratio_sigma-0.01.pdf}&
\includegraphics[height=\utilheightb]{figures/Pong_stepwise_ratio_sigma-0.03.pdf}&
\includegraphics[height=\utilheightb]{figures/Pong_stepwise_ratio_sigma-0.05.pdf}&
\includegraphics[height=\utilheightb]{figures/Pong_stepwise_ratio_sigma-0.1.pdf}\\[-1.2ex]
        & \makecell{\tiny{radius $r$}}
        & \makecell{\tiny{radius $r$}}
        & \makecell{\tiny{radius $r$}}
        & \makecell{\tiny{radius $r$}}
        & \makecell{\tiny{radius $r$}}
        & \makecell{\tiny{radius $r$}}
\end{tabular}
}
% \caption{\small Certified ratio $\eta_R$ w.r.t. radius $r$}\label{tab:cert-ratio}
\end{subtable}
}
\caption{\small Robustness certification for \textit{per-state action} in terms of certified ratio $\eta_r$ w.r.t. certified radius $r$. 
Each column corresponds to one smoothing parameter $\sigma$. The shaded area represents the standard deviation.
}%
\label{fig:cert-ratio}
\vspace{-2mm}
\end{figure}


==> [ICLR2022] robust-RL-CROP/fig_desc/fig_clean_full.tex <==
\newlength{\wrapheightb}
\settoheight{\wrapheightb}{\includegraphics[width=.40\textwidth]{figures/Freeway_clean_full.pdf}}%



\begin{wrapfigure}{r}{0.40\textwidth}
\vspace{-7mm}
\begin{center}
\includegraphics[height=\wrapheightb]{figures/Freeway_loact_clean_full.pdf}
\end{center}
\vspace{-5mm}
\caption{\small Benign performance of  locally smoothed policy $\tpi$ under a larger range of smoothing parameter $\sigma$ with clean state observations.}\label{fig:clean-full}
\end{wrapfigure}



==> [ICLR2022] robust-RL-CROP/fig_desc/fig_global.tex <==
{
\renewcommand{\thesubfigure}{\alph{subfigure}}
% {\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}

\begin{figure}



\newlength{\utilheightc}
\settoheight{\utilheightc}{\includegraphics[width=.155\linewidth]{figures/Freeway_global_mean_sigma-0.001.pdf}}%

\newlength{\utilheightd}
\settoheight{\utilheightd}{\includegraphics[width=.155\linewidth]{figures/Freeway_global_median_sigma-0.001.pdf}}%


\newlength{\utilheightaa}
\settoheight{\utilheightaa}{\includegraphics[width=.155\linewidth]{figures/Freeway_adasearch_sigma-0.001.pdf}}%

\newlength{\utilheightab}
\settoheight{\utilheightab}{\includegraphics[width=.155\linewidth]{figures/Pong_adasearch_sigma-0.001.pdf}}%

% \newlength{\utilheight}
% \settoheight{\utilheight}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: low degree.pdf}}%

% \newlength{\attackheightb}
% \settoheight{\attackheightb}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: high degree.pdf}}%

\newlength{\legendheightb}
\setlength{\legendheightb}{0.3\utilheightc}%


\newcommand{\rownamec}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightc][c]{\footnotesize #1}}}

\newcommand{\rownamed}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightd][c]{\footnotesize #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightb]{figures/legend.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\footnotesize{$\sigma=0.005$}}
        & \makecell{\footnotesize{$\sigma=0.05$}}
        & \makecell{\footnotesize{$\sigma=0.1$}}
        & \makecell{\footnotesize{$\sigma=0.5$}}
        & \makecell{\footnotesize{$\sigma=0.75$}}
        & \makecell{\footnotesize{$\sigma=1.0$}}
        \vspace{-1.7pt}\\
\rownamec{\makecell{Freeway}}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.005.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.01.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.05.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.1.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.5.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.75.pdf}\\[-1.2ex]
\rownamec{\makecell{Pong}}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.001.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.005.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.01.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.05.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.1.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.1.pdf}\\[-1.2ex]
\end{tabular}
% }
\caption{\small Expectation bound $\uje$: lower bound of $\ujefull$ w.r.t. $\eps$}\label{tab:ebound}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\rownamed{\makecell{Freeway}}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.005.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.01.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.05.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.1.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.5.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.75.pdf}\\[-1.2ex]
\rownamed{\makecell{Pong}}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.001.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.005.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.01.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.05.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.1.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.1.pdf}\\[-1.2ex]
\end{tabular}
% }
\caption{\small Percentile bound $\ujp$: lower bound of the $p$-th percentile of $\jfull$ w.r.t. $\eps$, with $p=50\%$}\label{tab:pbound}
\end{subtable}


\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\rownamed{\makecell{Freeway}}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.005.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.05.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.1.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.5.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.75.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-1.0.pdf}\\[-1.2ex]
\rownamed{\makecell{Pong}}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.001.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.005.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.01.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.03.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.05.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.1.pdf}\\[-1.2ex]
\end{tabular}
% }
\caption{\small Absolute lower bound $\uj$: lower bound of $\jfull$ w.r.t. $\eps$, with a given initial state}\label{tab:abound}
\end{subtable}

% \begin{subtable}[]{\linewidth}
% \centering
% % \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
% \rowname{\makecell{Freeway}}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.005.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.01.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.05.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.1.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.5.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.75.pdf}\\[-1.2ex]
% \rowname{\makecell{Pong}}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.001.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.005.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.01.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.05.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.1.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.5.pdf}\\[-1.2ex]
% \end{tabular}
% % }
% \caption{\small Certified ratio}\label{tab:cert-ratio}
% \end{subtable}
}
\caption{\small Certification for cumulative reward, including (a) expectation bound, (b) percentile bound, and (c) absolute lower bound for different models. Each column corresponds to one smoothing variance and each colored curve shows the result of one method as depicted in the legend.
\fan{Figures incomplete.}
}%
\label{fig:global-bound}
\end{figure}

}

==> [ICLR2022] robust-RL-CROP/fig_desc/fig_highway.tex <==
{
\renewcommand{\thesubfigure}{\alph{subfigure}}

\begin{figure}


% \newlength{\cputilheighta}
\settoheight{\cputilheighta}{\includegraphics[width=.160\linewidth]{figures/Freeway_stepwise_sigma-0.001.pdf}}%

% \newlength{\cpwrapheighta}
\settoheight{\cpwrapheighta}{\includegraphics[width=.400\textwidth]{figures/highway-fast_loact_clean.pdf}}%

% \newlength{\cplegendheight}
\setlength{\cplegendheight}{0.3\cputilheighta}%


\newcommand{\cprowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\cputilheighta][c]{\tiny #1}}}


% \newlength{\cputilheightc}
\settoheight{\cputilheightc}{\includegraphics[width=.160\linewidth]{figures/Freeway_global_mean_sigma-0.001.pdf}}%

% \newlength{\cputilheightd}
\settoheight{\cputilheightd}{\includegraphics[width=.165\linewidth]{figures/Freeway_global_median_sigma-0.001.pdf}}%


% \newlength{\cputilheightaa}
\settoheight{\cputilheightaa}{\includegraphics[width=.162\linewidth]{figures/Freeway_adasearch_sigma-0.05.pdf}}%

% \newlength{\cputilheightcp}
\settoheight{\cputilheightcp}{\includegraphics[width=.160\linewidth]{figures/highway-fast_global_mean_sigma-0.005.pdf}}%

% \newlength{\cputilheightdp}
\settoheight{\cputilheightdp}{\includegraphics[width=.165\linewidth]{figures/highway-fast_global_median_sigma-0.005.pdf}}%


% \newlength{\cputilheightaap}
\settoheight{\cputilheightaap}{\includegraphics[width=.162\linewidth]{figures/highway-fast_adasearch_sigma-0.75_cmp.pdf}}%


% % \newlength{\cputilheight}
% % \settoheight{\cputilheight}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: low degree.pdf}}%

% % \newlength{\attackheightb}
% % \settoheight{\attackheightb}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: high degree.pdf}}%

% \newlength{\cplegendheightb}
\setlength{\cplegendheightb}{0.3\cputilheightc}%


\newcommand{\cprownamec}[1]% #1 = text
{\rotatebox{90}{\makebox[\cputilheightc][c]{\tiny #1}}}

\newcommand{\cprownamed}[1]% #1 = text
{\rotatebox{90}{\makebox[\cputilheightd][c]{\tiny #1}}}



\centering



{
\renewcommand{\tabcolsep}{10pt}

\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\cplegendheight]{figures/Cartpole_legend.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\cprowname{\makecell{highway\\Radius $r$}}&
\includegraphics[height=\cputilheighta]{figures/highway-fast_stepwise_sigma-0.005.pdf}&
\includegraphics[height=\cputilheighta]{figures/highway-fast_stepwise_sigma-0.05.pdf}&
\includegraphics[height=\cputilheighta]{figures/highway-fast_stepwise_sigma-0.1.pdf}&
\includegraphics[height=\cputilheighta]{figures/highway-fast_stepwise_sigma-0.5.pdf}&
\includegraphics[height=\cputilheighta]{figures/highway-fast_stepwise_sigma-0.75.pdf}&
\includegraphics[height=\cputilheighta]{figures/highway-fast_stepwise_sigma-1.0.pdf}\\[-1.2ex]
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
\end{tabular}
\caption{\small Robustness certification for \textit{per-state action} in terms of certified radius $r$ at all time steps.
% We consider six methods: StdTrain, GaussAug, AdvTrain, RegPGD, RegCVX, and RadialRL, with the last three being SOTA. 
The shaded area represents the standard deviation.
% RadialRL is the most certifiably robust method on Freeway, while RegCVX is the most robust on CartPole.
}%
\label{fig:highway-statewise}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}


\begin{subtable}[]{\linewidth}
\centering
\includegraphics[height=\cpwrapheighta]{figures/highway-fast_loact_clean.pdf}
\vspace{-1mm}
\caption{\small Benign performance of  locally smoothed policy $\tpi$ under different  smoothing variance $\sigma$.}\label{fig:highway-statewise-clean}
\end{subtable}

\vspace{1em}

\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\cplegendheightb]{figures/CartPole_legend_marker.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{3mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\tiny{$\sigma=0.005$}}
        & \makecell{\tiny{$\sigma=0.05$}}
        & \makecell{\tiny{$\sigma=0.1$}}
        & \makecell{\tiny{$\sigma=0.5$}}
        & \makecell{\tiny{$\sigma=0.75$}}
        & \makecell{\tiny{$\sigma=1.0$}}
        \vspace{-1.7pt}\\
\cprownamec{\makecell{(Global) $\uje$}}&
\includegraphics[height=\cputilheightcp]{figures/highway-fast_global_mean_sigma-0.005.pdf}&
\includegraphics[height=\cputilheightcp]{figures/highway-fast_global_mean_sigma-0.05.pdf}&
\includegraphics[height=\cputilheightcp]{figures/highway-fast_global_mean_sigma-0.1.pdf}&
\includegraphics[height=\cputilheightcp]{figures/highway-fast_global_mean_sigma-0.5.pdf}&
\includegraphics[height=\cputilheightcp]{figures/highway-fast_global_mean_sigma-0.75.pdf}&
\includegraphics[height=\cputilheightcp]{figures/highway-fast_global_mean_sigma-1.0.pdf}\\[-1.2ex]
\cprownamed{\makecell{(Global) $\ujp$}}&
\includegraphics[height=\cputilheightdp]{figures/highway-fast_global_median_sigma-0.005.pdf}&
\includegraphics[height=\cputilheightdp]{figures/highway-fast_global_median_sigma-0.05.pdf}&
\includegraphics[height=\cputilheightdp]{figures/highway-fast_global_median_sigma-0.1.pdf}&
\includegraphics[height=\cputilheightdp]{figures/highway-fast_global_median_sigma-0.5.pdf}&
\includegraphics[height=\cputilheightdp]{figures/highway-fast_global_median_sigma-0.75.pdf}&
\includegraphics[height=\cputilheightdp]{figures/highway-fast_global_median_sigma-1.0.pdf}\\[-1.2ex]
\cprownamed{\makecell{(Local) $\uj$}}&
\includegraphics[height=\cputilheightaap]{figures/highway-fast_adasearch_sigma-0.005_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/highway-fast_adasearch_sigma-0.05_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/highway-fast_adasearch_sigma-0.1_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/highway-fast_adasearch_sigma-0.5_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/highway-fast_adasearch_sigma-0.75_cmp.pdf}&
\includegraphics[height=\cputilheightaap]{figures/highway-fast_adasearch_sigma-1.0_cmp.pdf}\\[-1.2ex]
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
\end{tabular}
}
\caption{\small Robustness certification as cumulative reward, including \textit{expectation bound} $\uje$, \textit{percentile bound} $\ujp$ ($p=50\%$), and \textit{absolute lower bound} $\uj$. 
% Each column corresponds to one smoothing variance. 
Solid lines represent the certified reward bounds of different methods, and dashed lines show the empirical performance under PGD attacks.}\label{tab:highway-bounds}
\end{subtable}
}

\caption{\small \textbf{Robustness certification on highway} in terms of (a-b): \textit{robustness of per-state action} and (c): \textit{lower bound of cumulative rewards}.
In (a) and (c), each column corresponds to one smoothing variance. 
% , including as cumulative reward, including \textit{expectation bound} $\uje$, \textit{percentile bound} $\ujp$ ($p=50\%$), and \textit{absolute lower bound} $\uj$  on (a) Freeway and (b) Pong. Each column corresponds to one smoothing variance. Solid lines represent the certified reward bounds of different methods, and dashed lines show the empirical performance under PGD attacks.
}\label{tab:highway-figs}
\end{figure}

}


==> [ICLR2022] robust-RL-CROP/fig_desc/fig_pong_periodic.tex <==
\begin{figure}[]
    \centering
    \begin{tabular}{c|c}
\includegraphics[width=.475\linewidth]{figures/pong-periodic-1.pdf}         &  \includegraphics[width=.475\linewidth]{figures/pong-periodic-2.pdf}
    \end{tabular}
    \caption{\small Periodic patterns in Pong. 
    The figure shows two periods (left and right), including the certified radius $r$ w.r.t. the time steps (above), and
    the selected game frames corresponding to different stages in each period (below).
    Different periods are highly similar.}
    \label{fig:pong-periodic}
\end{figure}

==> [ICLR2022] robust-RL-CROP/fig_desc/fig_reward.tex <==
{
\renewcommand{\thesubfigure}{\alph{subfigure}}
% {\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}

\begin{figure}
\vspace{-2em}


\newlength{\utilheightc}
\settoheight{\utilheightc}{\includegraphics[width=.160\linewidth]{figures/Freeway_global_mean_sigma-0.001.pdf}}%

\newlength{\utilheightd}
\settoheight{\utilheightd}{\includegraphics[width=.165\linewidth]{figures/Freeway_global_median_sigma-0.001.pdf}}%


\newlength{\utilheightaa}
\settoheight{\utilheightaa}{\includegraphics[width=.162\linewidth]{figures/Freeway_adasearch_sigma-0.05.pdf}}%

\newlength{\utilheightcp}
\settoheight{\utilheightcp}{\includegraphics[width=.160\linewidth]{figures/Pong_global_mean_sigma-0.001.pdf}}%

\newlength{\utilheightdp}
\settoheight{\utilheightdp}{\includegraphics[width=.165\linewidth]{figures/Pong_global_median_sigma-0.001.pdf}}%


\newlength{\utilheightaap}
\settoheight{\utilheightaap}{\includegraphics[width=.162\linewidth]{figures/Pong_adasearch_sigma-0.05.pdf}}%


% \newlength{\utilheight}
% \settoheight{\utilheight}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: low degree.pdf}}%

% \newlength{\attackheightb}
% \settoheight{\attackheightb}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: high degree.pdf}}%

\newlength{\legendheightb}
\setlength{\legendheightb}{0.48\utilheightc}%


\newcommand{\rownamec}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightc][c]{\tiny #1}}}

\newcommand{\rownamed}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightd][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=0.7\legendheightb]{figures/legend_marker.pdf}
\end{tabular}
\end{subtable}
\vspace{-2pt}
\begin{subtable}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{3mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\tiny{$\sigma=0.005$}}
        & \makecell{\tiny{$\sigma=0.05$}}
        & \makecell{\tiny{$\sigma=0.1$}}
        & \makecell{\tiny{$\sigma=0.5$}}
        & \makecell{\tiny{$\sigma=0.75$}}
        & \makecell{\tiny{$\sigma=1.0$}}
        \vspace{-2pt}\\
\rownamec{\makecell{(Global) $\uje$}}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.005_cmp.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.05_cmp.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.1_cmp.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.5_cmp.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.75_cmp.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-1.0_cmp.pdf}\\[-1.2ex]
\rownamed{\makecell{(Global) $\ujp$}}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.005_cmp.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.05_cmp.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.1_cmp.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.5_cmp.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.75_cmp.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-1.0_cmp.pdf}\\[-1.2ex]
\rownamed{\makecell{(Local) $\uj$}}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.005_cmp.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.05_cmp.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.1_cmp.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.5_cmp.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.75_cmp.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-1.0_cmp.pdf}\\[-1.2ex]
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
\end{tabular}
}
\vspace{-3mm}
\caption{\small Freeway}\label{tab:bound-freeway}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{3mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\tiny{$\sigma=0.001$}}
        & \makecell{\tiny{$\sigma=0.005$}}
        & \makecell{\tiny{$\sigma=0.01$}}
        & \makecell{\tiny{$\sigma=0.03$}}
        & \makecell{\tiny{$\sigma=0.05$}}
        & \makecell{\tiny{$\sigma=0.1$}}
        \vspace{-2pt}\\
\rownamec{\makecell{(Global) $\uje$}}&
\includegraphics[height=\utilheightcp]{figures/Pong_global_mean_sigma-0.001_cmp.pdf}&
\includegraphics[height=\utilheightcp]{figures/Pong_global_mean_sigma-0.005_cmp.pdf}&
\includegraphics[height=\utilheightcp]{figures/Pong_global_mean_sigma-0.01_cmp.pdf}&
\includegraphics[height=\utilheightcp]{figures/Pong_global_mean_sigma-0.03_cmp.pdf}&
\includegraphics[height=\utilheightcp]{figures/Pong_global_mean_sigma-0.05_cmp.pdf}&
\includegraphics[height=\utilheightcp]{figures/Pong_global_mean_sigma-0.1_cmp.pdf}\\[-1.2ex]
\rownamed{\makecell{(Global) $\ujp$}}&
\includegraphics[height=\utilheightdp]{figures/Pong_global_median_sigma-0.001_cmp.pdf}&
\includegraphics[height=\utilheightdp]{figures/Pong_global_median_sigma-0.005_cmp.pdf}&
\includegraphics[height=\utilheightdp]{figures/Pong_global_median_sigma-0.01_cmp.pdf}&
\includegraphics[height=\utilheightdp]{figures/Pong_global_median_sigma-0.03_cmp.pdf}&
\includegraphics[height=\utilheightdp]{figures/Pong_global_median_sigma-0.05_cmp.pdf}&
\includegraphics[height=\utilheightdp]{figures/Pong_global_median_sigma-0.1_cmp.pdf}\\[-1.2ex]
\rownamed{\makecell{(Local) $\uj$}}&
\includegraphics[height=\utilheightaap]{figures/Pong_adasearch_sigma-0.001_cmp.pdf}&
\includegraphics[height=\utilheightaap]{figures/Pong_adasearch_sigma-0.005_cmp.pdf}&
\includegraphics[height=\utilheightaap]{figures/Pong_adasearch_sigma-0.01_cmp.pdf}&
\includegraphics[height=\utilheightaap]{figures/Pong_adasearch_sigma-0.03_cmp.pdf}&
\includegraphics[height=\utilheightaap]{figures/Pong_adasearch_sigma-0.05_cmp.pdf}&
\includegraphics[height=\utilheightaap]{figures/Pong_adasearch_sigma-0.1_cmp.pdf}\\[-1.2ex]
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
\end{tabular}
}
\vspace{-3mm}
\caption{\small Pong}\label{tab:bound-pong}
\end{subtable}

% \begin{subtable}[]{\linewidth}
% \centering
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}p{3mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
%         & \makecell{\tiny{$\sigma=0.005$}}
%         & \makecell{\tiny{$\sigma=0.05$}}
%         & \makecell{\tiny{$\sigma=0.1$}}
%         & \makecell{\tiny{$\sigma=0.5$}}
%         & \makecell{\tiny{$\sigma=0.75$}}
%         & \makecell{\tiny{$\sigma=1.0$}}
%         \vspace{-2pt}\\
% \rownamec{\makecell{(Global) $\uje$}}&
% \includegraphics[height=\utilheightc]{figures/highway-fast_global_mean_sigma-0.005.pdf}&
% \includegraphics[height=\utilheightc]{figures/highway-fast_global_mean_sigma-0.05.pdf}&
% \includegraphics[height=\utilheightc]{figures/highway-fast_global_mean_sigma-0.1.pdf}&
% \includegraphics[height=\utilheightc]{figures/highway-fast_global_mean_sigma-0.5.pdf}&
% \includegraphics[height=\utilheightc]{figures/highway-fast_global_mean_sigma-0.75.pdf}&
% \includegraphics[height=\utilheightc]{figures/highway-fast_global_mean_sigma-1.0.pdf}\\[-1.2ex]
% \rownamed{\makecell{(Global) $\ujp$}}&
% \includegraphics[height=\utilheightd]{figures/highway-fast_global_median_sigma-0.005.pdf}&
% \includegraphics[height=\utilheightd]{figures/highway-fast_global_median_sigma-0.05.pdf}&
% \includegraphics[height=\utilheightd]{figures/highway-fast_global_median_sigma-0.1.pdf}&
% \includegraphics[height=\utilheightd]{figures/highway-fast_global_median_sigma-0.5.pdf}&
% \includegraphics[height=\utilheightd]{figures/highway-fast_global_median_sigma-0.75.pdf}&
% \includegraphics[height=\utilheightd]{figures/highway-fast_global_median_sigma-1.0.pdf}\\[-1.2ex]
% \rownamed{\makecell{(Local) $\uj$}}&
% \includegraphics[height=\utilheightaa]{figures/highway-fast_adasearch_sigma-0.005_cmp.pdf}&
% \includegraphics[height=\utilheightaa]{figures/highway-fast_adasearch_sigma-0.05_cmp.pdf}&
% \includegraphics[height=\utilheightaa]{figures/highway-fast_adasearch_sigma-0.1_cmp.pdf}&
% \includegraphics[height=\utilheightaa]{figures/highway-fast_adasearch_sigma-0.5_cmp.pdf}&
% \includegraphics[height=\utilheightaa]{figures/highway-fast_adasearch_sigma-0.75_cmp.pdf}&
% \includegraphics[height=\utilheightaa]{figures/highway-fast_adasearch_sigma-1.0_cmp.pdf}\\[-1.2ex]
%         & \makecell{\tiny{attack $\eps$}}
%         & \makecell{\tiny{attack $\eps$}}
%         & \makecell{\tiny{attack $\eps$}}
%         & \makecell{\tiny{attack $\eps$}}
%         & \makecell{\tiny{attack $\eps$}}
%         & \makecell{\tiny{attack $\eps$}}
% \end{tabular}
% }
% \vspace{-3mm}
% \caption{\small Highway}\label{tab:bound-highway-fast}
% \end{subtable}

}
\vspace{-3mm}
\caption{\small Robustness certification for cumulative reward, including \textit{expectation bound} $\uje$, \textit{percentile bound} $\ujp$ ($p=50\%$), and \textit{absolute lower bound} $\uj$. Each column corresponds to one smoothing variance. Solid lines represent the certified reward bounds, and dashed lines show the empirical performance under PGD.
% shows the change of the lower bounds w.r.t. the attack magnitude $\eps$.
% The solid curves represent the certified lower bounds, while the dotted lines represent the empirical values.
}%
\label{fig:all-bounds}
\vspace{-3em}
\end{figure}
}

==> [ICLR2022] robust-RL-CROP/fig_desc/fig_statewise.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}
\newcommand{\mycaption}[1]% #1 = caption
{\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}

\begin{figure}



\newlength{\utilheighta}
\settoheight{\utilheighta}{\includegraphics[width=.160\linewidth]{figures/Freeway_stepwise_sigma-0.001.pdf}}%


\newlength{\legendheight}
\setlength{\legendheight}{0.3\utilheighta}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheighta][c]{\tiny #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheight]{figures/legend.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\rowname{\makecell{Freeway\\Radius $r$}}&
\includegraphics[height=\utilheighta]{figures/Freeway_stepwise_sigma-0.005_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Freeway_stepwise_sigma-0.05_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Freeway_stepwise_sigma-0.1_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Freeway_stepwise_sigma-0.5_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Freeway_stepwise_sigma-0.75_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Freeway_stepwise_sigma-1.0_new.pdf}\\[-1.2ex]
\rowname{\makecell{Pong\\Radius $r$}}&
\includegraphics[height=\utilheighta]{figures/Pong_stepwise_sigma-0.001_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Pong_stepwise_sigma-0.005_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Pong_stepwise_sigma-0.01_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Pong_stepwise_sigma-0.03_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Pong_stepwise_sigma-0.05_new.pdf}&
\includegraphics[height=\utilheighta]{figures/Pong_stepwise_sigma-0.1_new.pdf}\\[-1.2ex]
% \rowname{\makecell{Highway\\Radius $r$}}&
% \includegraphics[height=\utilheighta]{figures/highway-fast_stepwise_sigma-0.005.pdf}&
% \includegraphics[height=\utilheighta]{figures/highway-fast_stepwise_sigma-0.05.pdf}&
% \includegraphics[height=\utilheighta]{figures/highway-fast_stepwise_sigma-0.1.pdf}&
% \includegraphics[height=\utilheighta]{figures/highway-fast_stepwise_sigma-0.5.pdf}&
% \includegraphics[height=\utilheighta]{figures/highway-fast_stepwise_sigma-0.75.pdf}&
% \includegraphics[height=\utilheighta]{figures/highway-fast_stepwise_sigma-1.0.pdf}\\[-1.2ex]
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small Robustness certification for \textit{per-state action} in terms of certified radius $r$ at all time steps.
Each column corresponds to a smoothing variance $\sigma$. 
% We consider six methods: StdTrain, GaussAug, AdvTrain, RegPGD, RegCVX, and RadialRL, with the last three being SOTA. 
The shaded area represents the standard deviation which is small.
RadialRL is the most certifiably robust method on Freeway, while SA-MDP (CVX) is the most robust on Pong.
}%
\label{fig:statewise}
\vspace{-2em}
\end{figure}



==> [ICLR2022] robust-RL-CROP/fig_desc/fig_statewise_clean.tex <==
\newlength{\wrapheighta}
\settoheight{\wrapheighta}{\includegraphics[width=.245\textwidth]{figures/Freeway_clean.pdf}}%



\begin{wrapfigure}{R}{0.63\linewidth}
\vspace{-7mm}
\begin{center}
\includegraphics[height=\wrapheighta]{figures/Freeway_loact_clean_new.pdf}
\includegraphics[height=\wrapheighta]{figures/Pong_loact_clean.pdf}
% \includegraphics[height=\wrapheighta]{figures/highway-fast_loact_clean.pdf}
\end{center}
\vspace{-5mm}
\caption{\small Benign performance of  locally smoothed policy $\tpi$ under different  smoothing variance $\sigma$ with clean state observations.}\label{fig:statewise-clean}
\vspace{-1em}
\end{wrapfigure}



==> [ICLR2022] robust-RL-CROP/fig_desc/fig_statewise_large.tex <==
\begin{figure}


\newlength{\utilheightlarge}
\settoheight{\utilheightlarge}{\includegraphics[width=.15\linewidth]{figures/Freeway_stepwise_sigma-1.5.pdf}}%


\newlength{\utilheightlargeada}
\settoheight{\utilheightlargeada}{\includegraphics[width=.15\linewidth]{figures/Freeway_adasearch_sigma-1.5.pdf}}%


\newlength{\legendheightlarge}
\setlength{\legendheightlarge}{0.4\utilheightlarge}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightlarge][c]{\tiny #1}}}


\centering

{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightlarge]{figures/legend_simp.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{0.48\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{3mm}@{}c@{}c@{}c@{}}
        & \makecell{\tiny{$\sigma=1.5$}}
        & \makecell{\tiny{$\sigma=2.0$}}
        & \makecell{\tiny{$\sigma=4.0$}}\\
\rowname{\makecell{Radius $r$}}&
\includegraphics[height=\utilheightlarge]{figures/Freeway_stepwise_sigma-1.5.pdf}&
\includegraphics[height=\utilheightlarge]{figures/Freeway_stepwise_sigma-2.0.pdf}&
\includegraphics[height=\utilheightlarge]{figures/Freeway_stepwise_sigma-4.0.pdf}\\[-1.2ex]
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
        & \makecell{\tiny{time step $t$}}
\end{tabular}
% }
\caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad-large}
\end{subtable}
\begin{subtable}[]{0.48\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{3mm}@{}c@{}c@{}c@{}}
        & \makecell{\tiny{$\sigma=1.5$}}
        & \makecell{\tiny{$\sigma=2.0$}}
        & \makecell{\tiny{$\sigma=4.0$}}\\
\rowname{\makecell{$\uj$}}&
\includegraphics[height=\utilheightlargeada]{figures/Freeway_adasearch_sigma-1.5.pdf}&
\includegraphics[height=\utilheightlargeada]{figures/Freeway_adasearch_sigma-2.0.pdf}&
\includegraphics[height=\utilheightlargeada]{figures/Freeway_adasearch_sigma-4.0.pdf}\\[-1.2ex]
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
        & \makecell{\tiny{attack $\eps$}}
\end{tabular}
% }
\caption{\small Absolute lower bound $\uj$ w.r.t. attack $\eps$}\label{tab:cert-uj-large}
\end{subtable}

}
\caption{\small Robustness certification for (a) \textit{per-state action} in terms of certified radius $r$ at all time steps, and (b) \textit{cumulative reward} in terms of absolute lower bound $\uj$ w.r.t. the attack magnitude $\eps$. The results are reported under large smoothing parameter $\sigma$ compared with those evaluated in~\Cref{fig:statewise} and~\Cref{fig:all-bounds} in the main paper.
% Each column corresponds to one smoothing variance $\sigma$. 
% We consider six methods: StdTrain, GaussAug, AdvTrain, RegPGD, RegCVX, and RadialRL, with the last three being SOTA. 
% The shaded area represents the standard deviation which is small.
% RadialRL is the most certifiably robust method on Freeway, while RegCVX is the most robust on Pong.
}%
\label{fig:statewise-large}
\vspace{-1em}
\end{figure}



==> [ICLR2022] robust-RL-CROP/macro.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bo}[1]{\textcolor{blue}{(Bo: #1)}}
\newcommand{\fan}[1]{{\color{orange!90!black}(Fan: #1)}}
\newcommand{\fanm}[1]{{\color{orange!90!black}#1}}
\newcommand{\tx}[1]{{\color{violet}(Tengyang: #1)}}
\newcommand{\linyi}[1]{{\color{olive}(Linyi: #1)}}
\newcommand{\linyim}[1]{{\color{olive}#1}}
% \newcommand{\cz}[1]{{\color{red} #1}}
\newcommand{\mo}[1]{{\color{blue}#1}}


\newcommand{\more}[0]{{\color{orange}..................}}


\usepackage{soul}
\usepackage[normalem]{ulem}
\renewcommand\sout{\bgroup\markoverwith
{\color{orange!90!black}{\rule[.5ex]{2pt}{1pt}}}\ULon}



\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}


\newcommand*{\commentfont}{\fontsize{\tiny}\selectfont}


% % \numberwithin{equation}{section}

% \usepackage{bbm}


% % \usepackage{fancyhdr}
\usepackage{graphicx}
\usepackage{xcolor}


\usepackage{multicol}

% \usepackage{algorithm} 
\usepackage{algorithmic}  
% \usepackage[algo2e]{algorithm2e} 
% \usepackage{algorithm}
% % \usepackage{algorithmic}

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}
\usepackage{adjustbox}
\SetKwComment{Comment}{$\triangleright$\ }{}





\usepackage{nicefrac}




% enumerate
\usepackage[shortlabels]{enumitem}


% \usepackage[margin=1in]{geometry}
\usepackage{hyperref}
\usepackage[nameinlink]{cleveref}
\crefname{ineq}{inequality}{inequalities}
\creflabelformat{ineq}{#2{\upshape(#1)}#3} 

\usepackage{longtable}

\usepackage{amsthm}


\usepackage{bbm}
\usepackage{dsfont}







\newcommand{\brows}[1]{%
  \begin{bmatrix}
  \begin{array}{c}
  #1
  \end{array}
  \end{bmatrix}
}
\newcommand{\rotvert}{\rotatebox[origin=c]{90}{$\vert$}}
\newcommand{\rowsvdots}{\multicolumn{1}{@{}c@{}}{\vdots}}


% for 1st, 2nd, 3th...
\usepackage[super]{nth}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% definitions and theorems
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\theoremstyle{plain}
\newtheorem{theoremappend}{Theorem}
\theoremstyle{plain}
% \newtheorem{lemma}{Lemma}
\theoremstyle{plain}
\newtheorem{prop}{Proposition}


\usepackage{thmtools}
\usepackage{thm-restate}

\theoremstyle{plain}
\declaretheorem[name=Theorem]{theorem}
\theoremstyle{plain}
\declaretheorem[name=Lemma]{lemma}


% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{corollary}[theorem]{Corollary}
% % \theoremstyle{definition}
% \newtheorem{definition}{Definition}
% \newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}
% \newtheorem{conjecture}{Conjecture}


% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{corollary}{Corollary}[theorem]
% \newtheorem{lemma}[theorem]{Lemma}

% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]


% % inline math allow break
% \makeatletter
% \def\old@comma{,}
% \catcode`\,=13
% \def,{%
%   \ifmmode%
%     \old@comma\discretionary{}{}{}%
%   \else%
%     \old@comma%
%   \fi%
% }
% \makeatother



% new commands
\newcommand{\eg}[0]{\textit{e.g.}}
\newcommand{\etal}[0]{\textit{et al.}\xspace}
\newcommand{\resp}[0]{\textit{resp.}}
\newcommand{\ie}[0]{\textit{i.e.}}
% \newcommand{\st}[0]{\textit{s.t.}\xspace}
\renewcommand{\wp}[0]{\textit{w.p.}\xspace}
\newcommand{\ow}[0]{\textit{o.w.}\xspace}
\newcommand{\wrt}[0]{\textit{w.r.t.}\xspace}
\newcommand{\eps}[0]{\varepsilon}
\newcommand{\lmb}[0]{\lambda}
\newcommand{\cov}[0]{\mbox{Cov}}
\newcommand{\Exp}[0]{\mbox{Exp}}
\newcommand{\var}[0]{\mbox{var}}
\newcommand{\aeq}[0]{\stackrel{\cdot}{=}}

\newcommand{\wtilde}[0]{\widetilde}
\newcommand{\wbar}[0]{\widebar}


\newcommand{\namepertmag}[0]{maximum perturbation magnitude\xspace}

\newcommand{\namef}[0]{perturbed return function\xspace}
\newcommand{\nameF}[0]{Perturbed return function\xspace}

\newcommand{\namej}[0]{finite horizon cumulative reward\xspace}
\newcommand{\namepj}[0]{perturbed cumulative reward\xspace}


\newcommand{\ebound}[0]{expectation bound\xspace}
\newcommand{\pbound}[0]{percentile bound\xspace}

\newcommand{\sigrtj}[0]{$\sigma$-randomized trajectory\xspace}
\newcommand{\sigrtjs}[0]{$\sigma$-randomized trajectories\xspace}
\newcommand{\sigrpi}[0]{$\sigma$-randomized policy\xspace}


\usepackage{accents}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\uit}[1]{\underline{\textit{#1}}}
\newcommand{\texttc}[1]{\texttt{\textsc{#1}}}


\newcommand{\dtv}[0]{\mathrm{D}_{\mathrm{TV}}}

\newcommand{\rzero}[0]{\rightarrow0}
\newcommand{\rinf}[0]{\rightarrow\infty}
\newcommand{\smax}[0]{\scriptsize \mbox{max}}
\newcommand{\smin}[0]{\scriptsize \mbox{min}}


\newcommand{\Eop}{\mathop{\mathbb E}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% project specific macros
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\RL}[0]{Reinforcement Learning\xspace}
\newcommand{\rl}[0]{reinforcement learning\xspace}
\newcommand{\lip}[0]{Lipschitz\xspace}
\newcommand{\env}[0]{environment\xspace}   
\newcommand{\qpi}[0]{Q^\pi}
\newcommand{\tpi}[0]{\tilde\pi}
\newcommand{\wqpi}[0]{\wtilde Q^\pi}

\newcommand{\vmin}[0]{V_{\min}}
\newcommand{\vmax}[0]{V_{\max}}
\newcommand{\jmin}[0]{J_{\min}}
\newcommand{\jmax}[0]{J_{\max}}
\newcommand{\jcur}[0]{J_{\rm cur}}
\newcommand{\jglobal}[0]{J_{\rm global}}
\newcommand{\sm}[0]{\cal S_{\rm{m}}^\eps}
\newcommand{\epsball}[0]{\cal B^\eps}
\newcommand{\epsbball}[0]{\cal B^{\bar\eps}}

\renewcommand{\vert}[0]{\oplus}
\newcommand{\vertt}[2]{\vert_{t=#1}^{#2}}


\newcommand{\uj}[0]{\underline{J}}
\newcommand{\uje}[0]{\underline{J_E}}
\newcommand{\ujp}[0]{\underline{J_p}}

\newcommand{\ujefull}[0]{E\left[J_\eps^H(\pi')\right]}
\newcommand{\jfull}[0]{J_\eps^H(\pi')}





% \newcommand{\staters}[0]{\textsc{LocalRS-Act}\xspace}
% \newcommand{\glbrs}[0]{\textsc{GlobalRS-CR}\xspace}
% \newcommand{\adasearch}[0]{\textsc{LocalRS-CR}\xspace}

\newcommand{\sysname}[0]{\textsc{CROP}\xspace}

\newcommand{\staters}[0]{\textsc{\sysname-LoAct}\xspace}
\newcommand{\glbrs}[0]{\textsc{\sysname-GRe}\xspace}
\newcommand{\adasearch}[0]{\textsc{\sysname-LoRe}\xspace}



\newcommand{\norm}[1]{\lVert{#1}\rVert}
\newcommand{\dotp}[2]{\langle {#1},{#2} \rangle}
\newcommand{\bb}[1]{\mathbb{#1}}
\newcommand{\bbm}[1]{\mathbbm{#1}}


\newcommand{\pmat}[2]{
                    \begin{pmatrix}
                    #1\\#2
                    \end{pmatrix}
                    }
\newcommand{\intt}[2]{\int_{#1}^{#2}}
\renewcommand{\cal}[1]{\mathcal{#1}}
% \renewcommand{\bf}[1]{\mathbf{#1}}
\newcommand{\tbf}[1]{{\textbf{#1}}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% spacing (blank space)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{float}
% \setlength{\textfloatsep}{0.2cm}

\setlength{\abovedisplayskip}{-20pt}
\setlength{\belowdisplayskip}{-20pt}
\setlength{\abovedisplayshortskip}{-20pt}
\setlength{\belowdisplayshortskip}{-20pt}


\usepackage{titlesec}
\titlespacing{\section}{0pt}{6pt}{6pt}
\titlespacing{\subsection}{0pt}{6pt}{6pt}



% \titlespacing*{\section}
% {0pt}{2.5ex plus 0.5ex minus .2ex}{4.3ex plus .2ex}
% \titlespacing*{\subsection}
% {0pt}{2.5ex plus 0.5ex minus .2ex}{4.3ex plus .2ex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% tables and figures
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \usepackage{float}
% \setlength{\textfloatsep}{0.1cm}

\usepackage{subcaption}

\usepackage{booktabs}
\usepackage{makecell}


\usepackage{wrapfig}

% \newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
% \newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
% \newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
% \newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}

\newcommand\given[1][]{\:#1\vert\:}


% \makeatletter
% \newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\ignorespaces\fi}
% \makeatother


\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\ignorespaces\fi}
\makeatother





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% widebar
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother

==> [ICLR2022] robust-RL-CROP/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> [ICLR2022] robust-RL-CROP/pseudo-code/adaptive-search-main.tex <==
% \begin{algorithm}[t]
% \algsetup{linenosize=\tiny}
% \scriptsize
% \DontPrintSemicolon
% \setlength{\columnsep}{15pt}
% \begin{multicols}{2}
% \KwIn{initial state distribution $d_0$, deterministic transition function $\Gamma(s,a)$, deterministic immediate reward function $R(s,a)$, trained value network $Q^\pi$ with range $[\vmin, \vmax]$; parameters for randomized smoothing: sampling times $m$, smoothing variance $\sigma^2$, one-sided confidence parameter $\alpha$}
% \KwOut{a map $M$ that maps a radius $R$ to the corresponding certified lower bound of reward $J$}
% \SetKwFunction{funca}{get\_action}
% \SetKwFunction{funcb}{expand}
% \SetKwProg{Pn}{Procedure}{:}{}
% \SetKwProg{Fn}{Function}{:}{}
% \Comment*[l]{\scriptsize Initialize global variables}
% $p\_que \leftarrow \emptyset$ \Comment*[r]{\tiny initialize an empty priority queue containing tuples of (state $s$, action $a$, radius $R$, reward $J$), sorted by increasing $R$}
% $M \leftarrow \emptyset$\; % \Comment*[r]{\tiny initialize an empty map that maps a radius $R$ to the certified lower bound of reward $J$}
% $\jglobal \leftarrow \infty$ \Comment*[r]{\tiny initialize global minimum reward}
% $\Delta =  \left( V_{\max} - V_{\min}\right) \sqrt{\frac{1}{2m} \ln \frac{1}{\alpha}}$ \Comment*[r]{\tiny confidence bound}\;

% \Fn{\funca{$s,\eps_{\rm lim}, \jcur$}}{
%     Generate noise samples $\delta_i\sim \cal N(0, \sigma^2I)$ for $1\leq i\leq m$\; 
%     \For {each action $a\in \cal A$} {
%         $\wtilde Q^\pi(s,a)\leftarrow \frac{1}{m} \sum_{i=1}^{m}\texttt{clip}( Q^\pi(s+\delta_i, a), \min=V_{\min}, \max=V_{\max})$\;
%     }
%     $a^\star\leftarrow \argmax_{a\in\cal A} \wtilde Q^\pi(s,a)$\;
%     $a\_list\leftarrow \emptyset$\;
%     \For {each action $a\in \cal A$} {
%         \If {$\Gamma(s,a)=\bot$} {
%             \textbf{continue}\;
%         }
%         % $re\leftarrow \jcur + R(s,a)$\;
%         \uIf {$\wtilde Q^\pi(s,a^\star) \geq \wtilde Q^\pi(s,a)+2\Delta$} {
%             $R\leftarrow \frac{\sigma}{2}(
%                                                 \Phi^{-1}(\frac{\wtilde Q^\pi(s,a^\star)-\Delta-V_{\min}}{V_{\max}-V_{\min}})-
%                                                 \Phi^{-1}(\frac{\wtilde Q^\pi(s,a)+\Delta-V_{\min}}{V_{\max}-V_{\min}})
%                                             )$\;
%         }
%         \Else {
%             $R \leftarrow $ 0\;
%         }
        
%         \uIf{$R\leq \eps_{\rm lim}$} { \Comment*[r]{\tiny take the possible action within $\eps_{\rm lim}$}
%             $a\_list\leftarrow a\_list \cup \{a\}$ 
%         }
%         \Else { \Comment*[r]{\tiny put currently impossible actions in queue for later expansion}
%             $p\_que.\texttt{push}((s, a, R, \jcur))$ 
%         }
%     }
%     \KwRet{$a\_list$}\;
% }
% \;
% \Pn{\funcb{$s,\eps_{\rm lim}, \jcur$}}{
%     \If {$\jcur \geq \jglobal$} {
%         \KwRet{$0$} \Comment*[r]{\tiny pruning}
%     }
%     $a\_list \leftarrow \funca(s,\eps_{\rm lim}, \jcur)$\;
%     \If {$a\_list = \emptyset$} {
%         $\jglobal \leftarrow \texttt{min}(\jglobal, \jcur)$\;
%         \KwRet{$0$}\;
%     }
%     \For {$a \in a\_list$} {
%         $s'\leftarrow \Gamma(s,a)$\;
%         $ret\leftarrow \funcb(s',\eps_{\rm lim}, \jcur+R(s,a))$\;
%     }
% }
% \;
% $s_0\sim d_0$ \Comment*[r]{\tiny initialize initial state}
% \funcb($s_0, \eps_{\rm lim}=0,\jcur=0$) \Comment*[r]{\tiny expand initial trajectory}
% \While {True} {
%     \If {$p\_que = \emptyset$} {
%         \textbf{break}\;
%     }
%     $(s,a,R,re)\leftarrow p\_que.\texttt{pop}()$ \Comment*[r]{\tiny pop out the first element of the priority queue}
%     $M[R] \leftarrow \jglobal$ \Comment*[r]{\tiny the certified lower bound of reward at $R$ is $\jglobal$}
%     $(s',a',R',re')\leftarrow p\_que.\texttt{top}()$ \Comment*[r]{\tiny examine the first element of the updated priority queue}
%     \funcb$(\Gamma(s,a), R', re+R(s,a))$ \Comment*[r]{\tiny expand the tree from the new state}
% }
% \end{multicols}
% \caption{\adasearch: Adaptive Search}\label{alg:adaptive-search}
% \end{algorithm}



% \newsavebox{\tempbox}


% \savebox{\tempbox}{% create image
% \begin{minipage}[c]{0.46\textwidth}%
\begin{algorithm}[t]
\algsetup{linenosize=\scriptsize}
\scriptsize
\DontPrintSemicolon
\setlength{\columnsep}{15pt}
\begin{multicols}{2}
% \setlength{\columnsep}{15pt}
\KwIn{Enivronment $\cal E=(\cal S, \cal A, R, \Gamma,d_0)$,
% initial state distribution $d_0$, deterministic transition function $\Gamma(s,a)$, deterministic immediate reward function $R(s,a)$, 
trained value network $Q^\pi$ with range $[\vmin, \vmax]$; parameters for randomized smoothing: sampling times $m$, smoothing variance $\sigma^2$, one-sided confidence parameter $\alpha$}
\KwOut{a map $M$ that maps an attack magnitude $\eps$ to the corresponding certified lower bound of reward $J$}
\SetKwFunction{funca}{\textsc{GetActions}}
\SetKwFunction{funcb}{\textsc{Expand}}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\Comment*[l]{\scriptsize Initialize global variables}
$p\_que \leftarrow \emptyset$ \Comment*[r]{\tiny initialize an empty priority queue containing tuples of (state $s$, action $a$, radius $r$, reward $J$), sorted by increasing $r$}
$M \leftarrow \emptyset$\; % \Comment*[r]{\tiny initialize an empty map that maps a radius $r$ to the certified lower bound of reward $J$}
$\jglobal \leftarrow \infty$ \Comment*[r]{\tiny initialize global minimum reward}
$\Delta =  \left( V_{\max} - V_{\min}\right) \sqrt{\frac{1}{2m} \ln \frac{1}{\alpha}}$ \Comment*[r]{\tiny confidence bound}\;

\Fn{\funca{$s,\eps_{\rm lim}, \jcur$}}{
    Generate noise samples $\delta_i\sim \cal N(0, \sigma^2I)$ for $1\leq i\leq m$\; 
    \For {each action $a\in \cal A$} {
        $\wtilde Q^\pi(s,a)\leftarrow \frac{1}{m} \sum_{i=1}^{m}\texttt{clip}( Q^\pi(s+\delta_i, a), \min=V_{\min}, \max=V_{\max})$\;
    }
    $a^\star\leftarrow \argmax_{a\in\cal A} \wtilde Q^\pi(s,a)$\;
    $a\_list\leftarrow \emptyset$\;
    \For {each action $a\in \cal A$} {
        \If {$\Gamma(s,a)=\bot$} {
            \textbf{continue}\;
        }
        % $re\leftarrow \jcur + R(s,a)$\;
        \uIf {$\wtilde Q^\pi(s,a^\star) \geq \wtilde Q^\pi(s,a)+2\Delta$} {
            $r\leftarrow \frac{\sigma}{2}(
                                                \Phi^{-1}(\frac{\wtilde Q^\pi(s,a^\star)-\Delta-V_{\min}}{V_{\max}-V_{\min}})-
                                                \Phi^{-1}(\frac{\wtilde Q^\pi(s,a)+\Delta-V_{\min}}{V_{\max}-V_{\min}})
                                            )$\;
        }
        \Else {
            $r\leftarrow $ 0\;
        }
        
        \uIf{$r\leq \eps_{\rm lim}$} { \Comment*[r]{\tiny take possible actions}
            $a\_list\leftarrow a\_list \cup \{a\}$ 
        }
        \Else { \Comment*[r]{\tiny store impossible actions in queue for later expansion}
            $p\_que.\texttt{push}((s, a, r, \jcur))$ 
        }
    }
    \KwRet{$a\_list$}\;
}
\;
\Pn{\funcb{$s,\eps_{\rm lim}, \jcur$}}{
    \If {$\jcur \geq \jglobal$} {
        \KwRet{$0$} \Comment*[r]{\tiny pruning}
    }
    $a\_list \leftarrow \funca(s,\eps_{\rm lim}, \jcur)$\;
    \If {$a\_list = \emptyset$} {
        $\jglobal \leftarrow \texttt{min}(\jglobal, \jcur)$\;
        \KwRet{$0$}\;
    }
    \For {$a \in a\_list$} {
        $s'\leftarrow \Gamma(s,a)$\;
        $ret\leftarrow \funcb(s',\eps_{\rm lim}, \jcur+R(s,a))$
    }
}
\;
$s_0\sim d_0$ \Comment*[r]{\tiny initialize initial state}
\funcb($s_0, \eps_{\rm lim}=0,\jcur=0$) \Comment*[r]{\tiny expand initial trajectory}
\While {True} {
    \If {$p\_que = \emptyset$} {
        \textbf{break}\;
    }
    \Comment*[r]{\tiny pop out the first element}
    $(s,a,r,J)\leftarrow p\_que.\texttt{pop}()$ \;
    \Comment*[r]{\tiny examine the next first element}
    $(\_,\_,r',\_)\leftarrow p\_que.\texttt{top}()$ \;
    \Comment*[r]{\tiny derive the critical $\eps$'s}
    $\eps \leftarrow r, \eps'\leftarrow r'$\;
    \Comment*[r]{\tiny obtain a pair of mapping}
    $M[\eps] \leftarrow \jglobal$ \;
    \Comment*[r]{\tiny expand the tree from the new node}
    \funcb$(\Gamma(s,a), \eps', J+R(s,a))$ 
}
\end{multicols}
\vspace{1em}
\caption{\adasearch: Adaptive search for certifying cumulative reward}\label{alg:adaptive-search-full}
\end{algorithm}%
% \end{minipage}
% }



% {
% \LinesNotNumbered
% \begin{algorithm}
% \LinesNotNumbered
% \caption{\adasearch: Adaptive search for certifying cumulative reward}\label{alg:adaptive-search}
% \clipbox{0pt {\depth} 0pt {\baselineskip}}{\usebox{\tempbox}}\hfill
% \raisebox{\depth}{\clipbox{0pt 1ex 0pt {\height}}{\usebox{\tempbox}}}
% \end{algorithm}
% }

==> [ICLR2022] robust-RL-CROP/pseudo-code/adaptive-search-skipframe.tex <==
\begin{algorithm}[t]
\algsetup{linenosize=\tiny}
\scriptsize
\DontPrintSemicolon
\KwIn{initial state distribution $d_0$, deterministic transition function $\Gamma(s,a)$, deterministic immediate reward function $r(s,a)$; trained value network $Q^\pi$; parameters for randomized smoothing: sampling times $m$, smoothing variance $\sigma^2$, one-sided confidence level parameter $\alpha$; frame skipping gap $k$}
\KwOut{a map $certify\_map$ that maps a radius $rad$ to the corresponding certified lower bound of reward $re$}
\SetKwFunction{funca}{get\_actions}
\SetKwFunction{funcb}{expand}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\Comment*[l]{\footnotesize Initialize global variables}
$p\_que \leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize an empty priority queue containing tuples of (state $s$, action $a$, radius $rad$, reward $re$) (sorted by increasing $rad$)}
$certify\_map \leftarrow \emptyset$\; % \Comment*[r]{\scriptsize initialize an empty map that maps a radius $rad$ to the certified lower bound of reward $re$}
$re\_min \leftarrow \infty$ \Comment*[r]{\scriptsize initialize global minimum reward}
$state\_set\leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize a set for visited states}
$state\_dict\leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize a map for visited states at current radius}
Generate noise samples $\delta_j\sim \cal N(0, \sigma^2I)$ for $1\leq j\leq m$\; 
$V_{\min}, V_{\max}\leftarrow$ sampled minimum and maximum value of the given network $Q^\pi$\;
$\Delta =  \left( V_{\max} - V_{\min}\right) \sqrt{\frac{1}{2m} \ln \frac{1}{\alpha}}$ \Comment*[r]{\scriptsize Hoeffding's bound under $\alpha$ confidence level}\;

\Fn{\funca{$s,a\_seq, rad\_lim, re\_cur$}}{
    $vis\leftarrow $ \texttt{False}\;
    \If { $s$ in $state\_set$ } {
        $vis\leftarrow $ \texttt{True}\;
    }
    $state\_set.\texttt{add}(s)$\;
    $k_s \leftarrow \texttt{len}(a\_seq)$\;
    $re\_accum \leftarrow 0$\;

    \For {$i$ from $1$ to $k_s-1$} { \Comment*[r]{\scriptsize skipping the first $k_s-1$ frames}
        $a \leftarrow a\_seq[i]$\;
        $re\_accum \leftarrow re\_accum + r(s, a)$\;
        $s \leftarrow \Gamma(s, a)$\;
        \If {$s = \bot$} {
            \KwRet $\bot, re\_accum$\;
        }
    }
    $a\_last \leftarrow a\_seq[k_s]$ \;
    $\wtilde Q^\pi(s,a) \leftarrow \frac{1}{m} \sum_{j=1}^{m}\texttt{clip}\left( Q^\pi(s+\delta_j, a), \min=V_{\min}, \max=V_{\max}\right)$\;
    $a^\star\leftarrow \argmax_{a\in\cal A} \wtilde Q^\pi(s,a)$\;
    % $re\leftarrow re\_cur + r(s,a)$\;
    \uIf {$\wtilde Q^\pi(s,a^\star) \geq \wtilde Q^\pi(s,a\_last)+2\Delta$} {
        $rad\leftarrow \frac{\sigma}{2}\left(
                                            \Phi^{-1}\left(\frac{\wtilde Q^\pi(s,a^\star)-\Delta-V_{\min}}{V_{\max}-V_{\min}}\right)-
                                            \Phi^{-1}\left(\frac{\wtilde Q^\pi(s,a)+\Delta-V_{\min}}{V_{\max}-V_{\min}}\right)
                                        \right)$\;
    }
    \Else {
        $rad \leftarrow $ 0\;
    }
    
    \uIf{$rad\leq rad\_lim$} {
        $re\_accum \leftarrow re\_accum + r(s, a\_last)$\;
        \KwRet $\Gamma(s, a\_last), re\_accum$ \Comment*[r]{\scriptsize take the possible action within $rad\_lim$}
    }
    \uElseIf {not $vis$} {
        $p\_que.\texttt{push}((s, a\_last, rad, re\_cur + re\_accum))$ \Comment*[r]{\scriptsize put currently impossible actions in queue}
        \KwRet $\texttt{Null}, re\_accum$\;
    }
}
\;
\Pn{\funcb{$s,rad\_lim, re\_cur$}}{
    \If {$re\_cur \geq re\_min$} {
        \KwRet{$0$} \Comment*[r]{\scriptsize pruning}
    }
    $k_s \leftarrow \min(k, estimated\_hit\_gap)$\;
    \Comment*[r]{\scriptsize estimate the time gap till the next frame where the ball hits the paddle}
    $a\_seq\_list \leftarrow \{[0,0,\ldots,0],
                                \underbrace{[1,0,\ldots,0],[1,1,\ldots,0],\ldots, [1,1,\ldots,1]}_{k_s \text{ sequences}},
                                \underbrace{[-1,0,\ldots,0],[-1,-1,\ldots,0],\ldots, [-1,-1,\ldots,-1]}_{k_s \text{ sequences}}\}$\;
    \Comment*[r]{\scriptsize $2k_s+1$ action sequences, where $\{-1,0,1\}$ means moving up / moving down / staying still}
    \For {$a\_seq \in a\_seq\_list$} {
        $s', re\_accum \leftarrow \funca{s, a\_seq, rad\_lim, re\_cur}$\;
        \uIf {$s' = \bot$} {
            $re\_min \leftarrow \min (re\_min, re\_cur + re\_accum)$\;
        }
        \uElseIf {$ s' \neq \texttt{Null}$} {
            \uIf {$s'$ in $state\_dict$} {
                $re\_ftr \leftarrow \min(re\_ftr, state\_dict[s'] + re\_accum)$\;
                $re\_min \leftarrow \min(re\_min, re\_cur + re\_accum)$\;
                % \textbf{continue}\;
            }
            \Else {
                $ret \leftarrow \funcb{s', rad\_lim, re\_cur + re\_accum} $\;
                $state\_dict[s'] \leftarrow \min(state\_dict[s'], ret)$\;
                $re\_ftr \leftarrow \min(re\_ftr, ret + re\_accum)$
            }
        }
    }
    \KwRet $re\_ftr$\;    
    % $a\_list \leftarrow \funca(s,rad\_lim, re\_cur)$\;
    % \If {$a\_list = \emptyset$} {
    %     $re\_min \leftarrow \texttt{min}(re\_min, re\_cur)$\;
    %     \KwRet{$0$}\;
    % }
    % $re\_ftr\leftarrow \infty$\;
    % \For {$a \in a\_list$} {
    %     $s'\leftarrow \Gamma(s,a)$\;
    %     \If { $s'$ in $state\_dict$ } {
    %         $re\_ftr\leftarrow\min(re\_ftr, state\_dict[s']+r(s,a))$\;
    %         $re\_min\leftarrow \min(re\_min, re\_cur+r(s,a))$\;
    %         \textbf{continue} \Comment*[r]{\scriptsize skip visited states}
    %     }
    %     $ret\leftarrow \funcb(s',rad\_lim, re\_cur+r(s,a))$\;
    %     $state\_dict[s'] = \min(state\_dict[s'], ret)$\;
    %     $re\_ftr\leftarrow \min(re\_ftr, ret+r(s,a))$\;
    % }
    % \KwRet{$re\_ftr$}\;
}
\;
$s_0\sim d_0$ \Comment*[r]{\scriptsize initialize initial state}
\funcb($s_0, rad\_lim=0,re\_cur=0$) \Comment*[r]{\scriptsize expand initial trajectory}
\While {True} {
    \If {$p\_que = \emptyset$} {
        \textbf{break}\;
    }
    $(s,a,rad,re)\leftarrow p\_que.\texttt{pop}()$ \Comment*[r]{\scriptsize pop out the first element of the priority queue}
    $state\_dict\leftarrow \emptyset$\;
    $certify\_map[rad] \leftarrow re\_min$ \Comment*[r]{\scriptsize the certified lower bound of reward at $rad$ is $re\_min$}
    $(s',a',rad',re')\leftarrow p\_que.\texttt{top}()$ \Comment*[r]{\scriptsize examine the first element of the updated priority queue}
    \funcb$(\Gamma(s,a), rad', re+r(s,a))$ \Comment*[r]{\scriptsize expand the tree from the new state}
}
\caption{Adaptive Search with Frame Skipping}\label{alg:adaptive-search}
\end{algorithm}



==> [ICLR2022] robust-RL-CROP/pseudo-code/adaptive-search.tex <==
\begin{algorithm}[!ht]
\algsetup{linenosize=\tiny}
\scriptsize
\DontPrintSemicolon
\KwIn{initial state distribution $d_0$, deterministic transition function $\Gamma(s,a)$, deterministic immediate reward function $r(s,a)$; trained value network $Q^\pi$; parameters for randomized smoothing: sampling times $m$, smoothing variance $\sigma^2$, one-sided confidence level parameter $\alpha$}
\KwOut{a map $certify\_map$ that maps a radius $rad$ to the corresponding certified lower bound of reward $re$}
\SetKwFunction{funca}{\textsc{GetAction}}
\SetKwFunction{funcb}{\textsc{Expand}}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\Comment*[l]{\footnotesize Initialize global variables}
$p\_que \leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize an empty priority queue containing tuples of (state $s$, action $a$, radius $rad$, reward $re$) (sorted by increasing $rad$)}
$certify\_map \leftarrow \emptyset$\; % \Comment*[r]{\scriptsize initialize an empty map that maps a radius $rad$ to the certified lower bound of reward $re$}
$re\_min \leftarrow \infty$ \Comment*[r]{\scriptsize initialize global minimum reward}
$state\_set\leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize a set for visited states}
$state\_dict\leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize a map for visited states at current radius}

$V_{\min}, V_{\max}\leftarrow$ sampled minimum and maximum value of the given network $Q^\pi$\;
$\Delta =  \left( V_{\max} - V_{\min}\right) \sqrt{\frac{1}{2m} \ln \frac{1}{\alpha}}$ \Comment*[r]{\scriptsize Hoeffding's bound under $\alpha$ confidence level}\;

\Fn{\funca{$s,rad\_lim, re\_cur$}}{
    $vis\leftarrow $ \texttt{False}\;
    \If { $s$ in $state\_set$ } {
        $vis\leftarrow $ \texttt{True}\;
    }
    $state\_set.\texttt{add}(s)$\;
    Generate noise samples $\delta_i\sim \cal N(0, \sigma^2I)$ for $1\leq i\leq m$\; 
    \For {each action $a\in \cal A$} {
        $\wtilde Q^\pi(s,a)\leftarrow \frac{1}{m} \sum_{i=1}^{m}\texttt{clip}\left( Q^\pi(s+\delta_i, a), \min=V_{\min}, \max=V_{\max}\right)$\;
    }
    $a^\star\leftarrow \argmax_{a\in\cal A} \wtilde Q^\pi(s,a)$\;
    $a\_list\leftarrow \emptyset$\;
    \For {each action $a\in \cal A$} {
        \If {$\Gamma(s,a)=\bot$} {
            \textbf{continue}\;
        }
        % $re\leftarrow re\_cur + r(s,a)$\;
        \uIf {$\wtilde Q^\pi(s,a^\star) \geq \wtilde Q^\pi(s,a)+2\Delta$} {
            $rad\leftarrow \frac{\sigma}{2}\left(
                                                \Phi^{-1}\left(\frac{\wtilde Q^\pi(s,a^\star)-\Delta-V_{\min}}{V_{\max}-V_{\min}}\right)-
                                                \Phi^{-1}\left(\frac{\wtilde Q^\pi(s,a)+\Delta-V_{\min}}{V_{\max}-V_{\min}}\right)
                                            \right)$\;
        }
        \Else {
            $rad \leftarrow $ 0\;
        }
        
        \uIf{$rad\leq rad\_lim$} {
            $a\_list\leftarrow a\_list \cup \{a\}$ \Comment*[r]{\scriptsize take the possible action within $rad\_lim$}
        }
        \uElseIf {not $vis$} {
            $p\_que.\texttt{push}((s, a, rad, re\_cur))$ \Comment*[r]{\scriptsize put currently impossible actions in queue for later expansion}
        }
    }
    \KwRet{$a\_list$}\;
}
\;
\Pn{\funcb{$s,rad\_lim, re\_cur$}}{
    \If {$re\_cur \geq re\_min$} {
        \KwRet{$0$} \Comment*[r]{\scriptsize pruning}
    }
    $a\_list \leftarrow \funca(s,rad\_lim, re\_cur)$\;
    \If {$a\_list = \emptyset$} {
        $re\_min \leftarrow \texttt{min}(re\_min, re\_cur)$\;
        \KwRet{$0$}\;
    }
    $re\_ftr\leftarrow \infty$\;
    \For {$a \in a\_list$} {
        $s'\leftarrow \Gamma(s,a)$\;
        \If { $s'$ in $state\_dict$ } {
            $re\_ftr\leftarrow\min(re\_ftr, state\_dict[s']+r(s,a))$\;
            $re\_min\leftarrow \min(re\_min, re\_cur+r(s,a))$\;
            \textbf{continue} \Comment*[r]{\scriptsize skip visited states}
        }
        $ret\leftarrow \funcb(s',rad\_lim, re\_cur+r(s,a))$\;
        $state\_dict[s'] = \min(state\_dict[s'], ret)$\;
        $re\_ftr\leftarrow \min(re\_ftr, ret+r(s,a))$\;
    }
    \KwRet{$re\_ftr$}\;
}
\;
$s_0\sim d_0$ \Comment*[r]{\scriptsize initialize initial state}
\funcb($s_0, rad\_lim=0,re\_cur=0$) \Comment*[r]{\scriptsize expand initial trajectory}
\While {True} {
    \If {$p\_que = \emptyset$} {
        \textbf{break}\;
    }
    $(s,a,rad,re)\leftarrow p\_que.\texttt{pop}()$ \Comment*[r]{\scriptsize pop out the first element of the priority queue}
    $state\_dict\leftarrow \emptyset$\;
    $certify\_map[rad] \leftarrow re\_min$ \Comment*[r]{\scriptsize the certified lower bound of reward at $rad$ is $re\_min$}
    $(s',a',rad',re')\leftarrow p\_que.\texttt{top}()$ \Comment*[r]{\scriptsize examine the first element of the updated priority queue}
    \funcb$(\Gamma(s,a), rad', re+r(s,a))$ \Comment*[r]{\scriptsize expand the tree from the new state}
}
\caption{\adasearch: Adaptive Search}\label{alg:adaptive-search-full}
\end{algorithm}



==> [ICLR2022] robust-RL-CROP/pseudo-code/gaussian-aug.tex <==
\begin{algorithm}[t]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
% \KwOut{action $a$}
\DontPrintSemicolon
Initialize replay buffer $D=\emptyset$\;
Initialize action-value function $Q$ with random weight $\theta$\;
Initialize target action-value function with weight $\theta^-=\theta$\;
\For {$episode=1$ to $M$}{
    Initialize state $s_1$\;
    % {\color{red}
    % \For {$t=1$ to $T$} {
    %     \For {$i=1$ to $n$} {
    %         $\eps_{ti}\leftarrow\cal N(0,\sigma^2)$\Comment*[r]{\scriptsize generate all perturbations beforehand}
    %     }
    % }
    % }
    \For {$t=1$ to $T$}{
        Following $\eps$-greedy policy, select $a_t=\arg\max_a Q(s_t,a;\theta)$ \wp $\eps$, or a random action otherwise\;
        Execute action $a_t$ and observe reward $r_t$ and next state $s_{t+1}$\;
        % {\color{red}
        % \For {$i=1$ to $n$}{
        %     \For {$j=1$ to $n$}{
        %         $\tilde s_t\leftarrow s_t+\eps_{t,i}$\;
        %         $\tilde s_{t+1}\leftarrow s_{t+1}+\eps_{t+1,j}$\;
        %         Store $(\tilde s_t,a_t,r_t,\tilde s_{t+1})$ in $D$ \Comment*[r]{\scriptsize store the smoothed transitions}
        %     }
        % }
        % }
        Sample random minibatch of transitions $(s_j,a_j,r_j,s_{j+1})$ from $D$ \Comment*[r]{\scriptsize Experience Replay}
        {\color{red}
        \Comment*[l]{\scriptsize Gaussian Data Augmentation}
        $\delta\leftarrow \cal N(0,\sigma^2)$ \;
        $\tilde s_j = s_j + \delta $\;
        $\tilde s_{j+1} = s_{j+1} + \delta $\;
        }
        $y_j\leftarrow r_j+\gamma \max_{a'}Q(\tilde s_{j+1},a';\theta^-)$\;
        Perform a gradient descent step on $(y_j-Q(\tilde s_j,a_j;\theta))^2$ \wrt the network parameter $\theta$\;
        Every $C$ steps set $\theta^-=\theta$ \Comment*[r]{\scriptsize Update the target network periodically}
    }
}
\caption{\textbf{[DQN]} Gaussian data augmentation during training}\label{alg:gaussian-augment}
\end{algorithm}


==> [ICLR2022] robust-RL-CROP/pseudo-code/global-certify.tex <==
\begin{algorithm}[t]
\algsetup{linenosize=\tiny}
\footnotesize
\DontPrintSemicolon
\setlength{\columnsep}{15pt}
\begin{multicols}{2}
\KwIn{initial state distribution $d_0$, trained value network $\qpi$, game cumulative reward range $[\jmin,\jmax]$, number of steps in an episode $H$, perturbation magnitude at each state $\eps$, percentile $p$; parameters for smoothing: sampling times $m$, smoothing variance $\sigma^2$, one-sided confidence parameter $\alpha$}
\KwOut{Expectation bound $\uje$, $p$-th percentile bound $\ujp$}
\Comment*[l]{\footnotesize Step 1: smoothing}
\For {$i=1$ to $m$} {
    $s_0\sim d_0, J^C_i\leftarrow 0$ \Comment*[r]{\scriptsize initialization}
    Generate macro-state noise $\delta_t\sim \cal N(0, \sigma^2 I)$ for $0\leq t < H$\;
    \For {$t=0$ to $H-1$} {
        $a_t\leftarrow \argmax_{a}Q(s_{t}+\delta_t, a)$\;
        Execute action $a_t$ and observe reward $re_t$ and next state $s_{t+1}$ \Comment*[r]{\scriptsize take a step}
        $J^C_i\leftarrow J^C_i + re_t$ \Comment*[r]{\scriptsize accumulate the reward}
    }
}

\Comment*[l]{\footnotesize Step 2.1: certifying expectation bound}
$\wtilde F\leftarrow \frac{1}{m}\sum_{i=1}^{m} J^C_i$ \Comment*[r]{\scriptsize smoothed actual reward}
$\Delta_{\rm{conf}} \leftarrow (R_{\max}-R_{\min})\sqrt{\frac{\ln(1/\alpha)}{2m}}$ \\\Comment*[r]{\scriptsize confidence interval}
$\Delta_{\rm{lip}} \leftarrow \frac{R_{\max}-R_{\min}}{\sigma}\sqrt{\frac{2}{\pi}} \cdot \eps \sqrt{H}$ \\\Comment*[r]{\scriptsize bound given by \lip continuity}
$\uje \leftarrow \wtilde F - \Delta_{\rm{conf}} - \Delta_{\rm{lip}}$\;

\;
\Comment*[l]{\footnotesize Step 2.2: certifying percentile bound}
$k \leftarrow \texttc{ComputeOrderStats}(\eps,\sigma,p,m,H)$\;
$\ujp \leftarrow $ $k$-th smallest value in $\{J^C_i\}_{i=1}^{m}$\;
\;
\KwRet $\uje, \ujp$
\end{multicols}
\vspace{1em}
\caption{\small \glbrs: Global smoothing for certifying cumulative reward}\label{alg:global-rand}
\end{algorithm}

==> [ICLR2022] robust-RL-CROP/pseudo-code/local-certify.tex <==
\begin{algorithm}[t]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
\KwIn{state $s$, trained value network $Q^\pi$, one-sided confidence bound $\alpha$}
\KwOut{smoothed value network $\wtilde Q^\pi$, selected action $a$, certification flag $cert$, certified radius $R$, local \lip constant $L_s$; parameters for randomized smoothing: sampling times $m$, smoothing variance $\sigma^2$}
% \KwOut{action $a$}
\DontPrintSemicolon
\SetKwFunction{funcpgd}{projected\_gradient\_descent}
\SetKwFunction{funca}{compute\_cert\_R}
\SetKwFunction{funcb}{satisfy}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\funcpgd{$s,\eps$}} {
    objective function 
    \begin{align*}
        J=\min_{\substack{s'\\\st\norm{s'-s}_2\leq \eps}}
                \Phi^{-1}\left(\frac{\widetilde{Q}\left(s, a_1\right)-\Delta-l_{\mathcal{N}(s')}}{u_{\mathcal{N}(s')}-l_{\mathcal{N}(s')}}\right)
                    -
                \Phi^{-1}\left(\frac{\widetilde{Q}\left(s, a_2\right)+\Delta-l_{\mathcal{N}(s')}}{u_{\mathcal{N}(s')}-l_{\mathcal{N}(s')}}\right),
    \end{align*}
    where $\Delta=\left(u_{\mathcal{N}(s')}-l_{\mathcal{N}(s')}\right)\sqrt{\frac{1}{2m} \ln \frac{1}{\alpha}}$\;
    \KwRet{J}
}\;

\Fn{\funca{$s,\eps$}} {
    $J = \texttt{projected\_gradient\_descent}(s, \eps)$\;
    \If {$J = -1$} {
        \KwRet{$-1$}
    }
    $cert\_R \leftarrow \frac{\sigma}{2}J$\;
    \KwRet{$cert\_R$}\;
}\;

\Fn{\funcb{$cert\_R, \eps$}} {
    \KwRet{$\eps \geq cert\_R$}\;
}\;

\Comment*[l]{\footnotesize Main loop: binary search for the smallest R that satisfies ineq. (\ref{eq:r-cond})}
$hi\leftarrow 1, low\leftarrow 10^{-7}$\;
\While {$hi-low\geq 10^{-6}$} {
    $mid = (hi + low) / 2$\;
    $cert\_R \leftarrow \texttt{compute\_cert\_R}(s, \eps=mid)$\;
    \uIf {$cert\_R == -1$ or $\texttt{satisfy}(cert\_R, mid)$} {
        $hi \leftarrow mid$\;
    }
    \Else {
        $low \leftarrow mid$\;
    }
}
$R\leftarrow mid$\;
\KwRet $\wtilde Q$, $a_1$, $cert$, $R$, $L_s$\;
\caption{\small 
local \lip based randomized smoothing on action value function, along with the certification at given state.
}\label{alg:local-smooth-q}
\end{algorithm}


==> [ICLR2022] robust-RL-CROP/pseudo-code/stepwise-certify.tex <==
\begin{algorithm}[H]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
\setlength{\columnsep}{15pt}
\begin{multicols}{2}
\KwIn{state $s$, trained value network $Q^\pi$ with range $[V_{\min},V_{\max}]$; parameters for smoothing: sampling times $m$, smoothing variance $\sigma^2$, one-sided confidence parameter $\alpha$}
\KwOut{smoothed value network $\wtilde Q^\pi$, selected action $a$, certification indicator $cert$, certified radius $r$ constant $L$}
\SetKwFunction{funca}{pre-processing}
\SetKwFunction{funcb}{take\_one\_step}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
% \KwOut{action $a$}
\DontPrintSemicolon

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% for computing only r
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \Pn{\funca{}} {
%     % \Comment*[l]{\footnotesize Preprocessing: given a trained $Q$ network, compute its output range and the \lip constant of its smoothed version}
%     Sample the input states and pass them to the given network $Q$ to compute the minimum value $V_{\min}$ and maximum value $V_{\max}$\;
%     $L=\frac{ V_{\max} - V_{\min} }{\sigma}\sqrt{\nicefrac{2}{\pi}}$\;
% }\;

% \Fn{\funcb{$s,\eps$}} {
    \Comment*[l]{\footnotesize Step 1: smoothing}
    Generate noise samples $\delta_i\sim\cal N(0,\sigma^2 I)$ for $1\leq i\leq m$\;
    \For {each action $a \in \cal A$} {\Comment*[r]{\scriptsize clipping and averaging}
        $\wtilde Q^\pi(s,a)\leftarrow \frac{1}{m}\sum_{i=1}^{m} \texttt{clip}( Q^\pi(s+\delta_i, a), \min=V_{\min}, \max=V_{\max})$
    }
    $a_1,a_2\leftarrow $ best action and runner-up action given by $\wqpi$\;
    
    \columnbreak
    
    \Comment*[l]{\footnotesize Step 2: certification}
    $\Delta =  \left( V_{\max} - V_{\min}\right) \sqrt{\frac{1}{2m} \ln \frac{1}{\alpha}}$ \\\Comment*[r]{\scriptsize confidence interval}
    
    \uIf {$\wqpi(s,a_1) \geq \wqpi(s,a_2) + 2\Delta$} {
        \Comment*[r]{\scriptsize certification success}
        $cert\leftarrow$ \texttt{True}\;
        $r \leftarrow \frac{\sigma}{2}(
                                            \Phi^{-1}(\frac{\wqpi(s,a_1) - \Delta -V_{\min}}{V_{\max}-V_{\min}})
                                            -
                                            \Phi^{-1}(\frac{\wqpi(s,a_2) + \Delta -V_{\min}}{V_{\max}-V_{\min}})
                                      )$\;
    }
    \Else {
        \Comment*[r]{\scriptsize certification failure}
        $cert\leftarrow$ \texttt{False}\;
        $r \leftarrow $ \texttt{undefined}\;
    }
    \KwRet $\wqpi$, $a_1$, $cert$, $r$\;
% }
\end{multicols}
\caption{\small \staters: Local smoothing for certifying per-state action
}\label{alg:smooth-q}
\end{algorithm}


==> [ICLR2022] robust-RL-CROP/tables/tab_Breakout_lore.tex <==
{
\setlength{\tabcolsep}{4pt} % column sep

\begin{table}[]
    \centering

    \caption{\small \mo{\textbf{Empirical cumulative reward obtained under attacks of different magnitudes.}
    We follow~\citet{zhang2021robust} and~\citet{oikarinen2020robust} to conduct PGD attacks.
    We evaluate the trajectory length $H=200$. Each column group corresponds to one smoothing parameter $\sigma$. 
    For each smoothing parameter $\sigma$, we evaluate four attack magnitudes $\eps$.
    Different rows show the achieved empirical cumulative reward of different methods.}
    }
    \label{tab:breakout-lore}



\resizebox{\linewidth}{!}{%
        \begin{tabular}{c cccc cccc cccc
}
    \toprule
    \bm{$\sigma$} &  \multicolumn{4}{c}{$0.005$}  &  \multicolumn{4}{c}{$0.01$} &  \multicolumn{4}{c}{$0.05$}\\
    \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
    % & \multicolumn{4}{c}{$\eps$}  &  \multicolumn{4}{c}{$\eps$} &  \multicolumn{4}{c}{$\eps$}\\ 
    \bm{$\eps$} &    \multicolumn{1}{c}{\small $5e-3$}  & \multicolumn{1}{c}{\makecell{\small $1e-2$}} & \multicolumn{1}{c}{\makecell{\small $5e-2$}} &  \multicolumn{1}{c}{\small $1e-1$} 
    &    \multicolumn{1}{c}{\small $5e-3$}  & \multicolumn{1}{c}{\makecell{\small $1e-2$}} & \multicolumn{1}{c}{\makecell{\small $5e-2$}} &  \multicolumn{1}{c}{\small $1e-1$}
    &    \multicolumn{1}{c}{\small $5e-3$}  & \multicolumn{1}{c}{\makecell{\small $1e-2$}} & \multicolumn{1}{c}{\makecell{\small $5e-2$}} &  \multicolumn{1}{c}{\small $1e-1$}
    \\\midrule
\textbf{ StdTrain } & 6 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\
\textbf{ GaussAug } & 6 & 5 & 5 & 1 & 6 & 5 & 5 & 1 & 0 & 0 & 0 & 0 \\
\textbf{ AdvTrain } & 6 & 6 & 0 & 0 & 7 & 7 & 0 & 0 & 0 & 0 & 0 & 0 \\
\textbf{ RegPGD } & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule \\
\end{tabular}
}

\vspace{-5mm}
\end{table}
}

==> [ICLR2022] robust-RL-CROP/tx_draft.tex <==
\section{Performance Guarantees}

This section provides results on certificated robustness against perturbation on observation. 

Notations:
\begin{itemize}
\item Original value function (class): $f(\cdot,\cdot) \in \Fcal$
\item Smoothed function class: $\ftilde \coloneqq f(s,a) \circ \Ncal(0,\sigma^2 I) = \E_{\varepsilon \sim \Ncal(0,\sigma I)} \left[ f(s + \varepsilon, a)\right]$. $\widetilde \Fcal \coloneqq \{f \circ \Ncal(0,\sigma^2 I); f \in \Fcal\}$.
\item $f_1(s) = \max_{a \in \Acal} f(s,a)$
\item $f_2(s) = \max_{a \in \Acal \setminus a_s} f(s,a)$, where $a_s = \argmax_{a \in \Acal} f(s,a)$
\end{itemize}





\paragraph{Value-Based Approaches}

We now provide guarantees for the following procedure:
\begin{enumerate}
\item Approximate $Q^\star$ by $\Qhat$ in a unperturbed environment.
\item Smooth $\Qhat$ by $\Qtilde \coloneqq \Qhat \circ \Ncal(0,\sigma^2 I)$.
\item Output the greedy policy of $\Qtilde$.
\end{enumerate}

\begin{lemma}
\label{lem:tildelips}
$\Qtilde$ is $\frac{V_{\max}}{\sigma}\sqrt{\nicefrac{2}{\pi}}$-Lipschitz.
\end{lemma}

\begin{theorem}
Let $f$ be an arbitrary $L$-Lipschitz function, $\pi_{f}$ be the greedy policy of $f$, $\nu_\varepsilon$ denote arbitrary $L^2$ bounded observation perturbation. Then
\begin{align*}
J(\pi_{f}) - J(\pi_{f} \circ \nu_\varepsilon) \leq
\end{align*}
\end{theorem}

\begin{proof}
We now consider $Q^{\pi_{f}}$ and $Q^{\pi_{f} \circ \nu_\varepsilon}$.

\begin{align*}
&~ Q^{\pi_{f}}(s,\pi_f) - Q^{\pi_{f}}(s,\pi_{f} \circ \nu_\varepsilon)
\\
\leq &~ Q^{\pi_{f}}(s,\pi_f) - Q^{\pi_{f}}(s + \nu_\varepsilon(s),\pi_{f} \circ \nu_\varepsilon) + L_Q \varepsilon   \\ \tag{$Q^{\pi_{f}}$ is $L_Q$-Lipschitz by the MDP assumption}
\\
\leq &~ Q^{\pi_{f}}(s,\pi_f) - Q^{\pi_{f}}(s + \nu_\varepsilon(s),\pi_{f} \circ \nu_\varepsilon) + L_Q \varepsilon
\end{align*}

% \tx{It is not sure if only using $L$-Lipschitz $f$ is a sufficient condition to guarantee certificated robustness. If we also have $f$ closed to $Q^{\pi_f}$ (which is roughly $f \approx Q^\star$), then we are good. But things without that may not be doable.}

% \tx{For example, consider an extreme case --- $f$ is a constant function. In this case, $\pi_f$ and $\pi_{f} \circ \nu_\varepsilon$ can be two totally different policies.}

\end{proof}


==> archive/smooth_policy.tex <==
\subsection{Randomized Smoothing on Policies}

% See Section 3.3, Theorem 5, and Theorem 6 in~\cite{zhang2021robust}.

\begin{definition}[percentile smoothing~\cite{chiang2020detection}]
\label{def:median-smooth}
Given $f:\bb R^d\rightarrow \bb R$ and $G\sim\cal N(0,\sigma^2I)$, the percentile smoothing of $f$ is defined as:
\begin{align*}
\tilde f_{p}(x)&=\sup \{y \in \mathbb{R} \mid \mathbb{P}[f(x+G) \leq y] \leq p\}
\end{align*}
\end{definition}

For each action dimension $\mu(a^i|s)$, we apply percentile smoothing in~\Cref{def:median-smooth} to get $\tilde\mu(a^i|s)$.

\begin{lemma}[\cite{chiang2020detection}]
\label{lem:median-smooth}
A percentile-smoothed function $h_p$ with adversarial perturbation $\delta$ can be bounded as
\begin{align*}
    {h}_{\underline p}(x) \leq h_{p}(x+\delta) \leq {h}_{\bar{p}}(x) \quad \forall\|\delta\|_{2}<\epsilon,
\end{align*}
where $\underline{p}:=\Phi\left(\Phi^{-1}(p)-\frac{\epsilon}{\sigma}\right)$ and $\bar{p}:=\Phi\left(\Phi^{-1}(p)+\frac{\epsilon}{\sigma}\right)$, with $\Phi$ being the standard Gaussian CDF.
\end{lemma}

According to Lemma~\ref{lem:median-smooth}, the output action of the smoothed policy network will be bounded under attack.

\begin{lemma}[\cite{zhang2021robust}]
\label{lem:v-bound-dtv}
Given a policy $\pi$ and its value function $V^\pi(s)$. Denote the value function under the state perturbation of $\nu_\eps$ as $V_\eps^\pi(s)$. For all $s\in \cal S$, we have
\begin{align*}
    V^{\pi}(s)-{V}_{\eps}^\pi(s) \leq \alpha \max _{s \in \mathcal{S}}  \dtv(\mu(\cdot \mid s), \mu(\cdot \mid s+\nu_\eps(s))),
\end{align*}
where $\dtv(\mu(\cdot| s), \mu(\cdot|s+\nu_\eps(s)))$ is the total variation distance between $\mu(\cdot|s)$ and $\mu(\cdot|s+\nu_\eps(s))$, 
and $\alpha\triangleq 2\left[1+\frac{\gamma}{(1-\gamma)^{2}}\right] \max _{\left(s, a, s^{\prime}\right) \in \mathcal{S} \times \mathcal{A} \times \mathcal{S}}\left|R\left(s, a, s^{\prime}\right)\right|$ is a constant that does not depend on $\pi$.
\end{lemma}

\begin{theorem}
\label{thm:dtv-mu}
\begin{align*}
    \dtv(\mu(\cdot \mid s), \mu(\cdot \mid s+\nu_\eps(s)))\le\sum\left(\tilde\mu_{\bar p}(a^i|s)-\tilde\mu_{\underline p}(a^i|s) \right)
\end{align*}
\end{theorem}
\begin{proof}
    Immediate from Lemma~\ref{lem:median-smooth}.
\end{proof}
Combining Lemma~\ref{lem:v-bound-dtv} and~\Cref{thm:dtv-mu}, we conclude that the performance gap of the smoothed policy $\tilde \mu$ under clean and perturbed test environment will be bounded.

\textbf{next step}: check whether there is a tighter bound than Lemma~\ref{lem:v-bound-dtv}.

==> archive/thm-global-smoothing.tex <==
        \begin{theorem}
            Let $\pi'=\pi(s+\Delta)$ where $\Delta \sim \gN(0,\sigma^2I_S)$, $J(\pi')$ is 
            
            When $\norm{\delta_i}_2\leq \eps$ for all $i$, 
            $\wtilde F(\delta_1^m, \delta_2^m,\ldots, \delta_H^m)$ is lower bounded by
            % $\wtilde F(0,0,\ldots,0)-(R_{\max}-R_{\min})\sqrt{\frac{\ln(1/\alpha)}{2m}} - L\eps\sqrt{H}$
            $\wtilde F(0,0,\ldots,0) - L\eps\sqrt{H}$.
            % with $m$ sampled macro-states and confidence parameter $\alpha$. 
            % $R_{\max}$ and $R_{\min}$ are the maximum and minimum cumulative reward of the game known a priori, and  
            $L$ is the \lip constant in~\Cref{lem:global-lip}.
        \end{theorem}

==> archive/thm-proof-radius.tex <==
\iffalse
\begin{proof}
We first present the bound for the smoothed value function $\wtilde V^\pi$. For each $s \in \cal S$, given the local \lip continuity of the smoothed $\wtilde Q^\pi$ (\Cref{lem:lipschitz}), we have
    \begin{align*}
        \wtilde V_\eps^\pi(s)-\wtilde V^\pi(s)
&=      \wtilde V^\pi (s + \nu_\eps(s)) - \wtilde V^\pi (s)\\
&=        \max_{a_1}\wtilde Q^\pi(s+\nu_\eps(s),a_1)-\max_{a_2}\wtilde Q^\pi(s,a_2)\\
&\geq     \wtilde Q^\pi(s+\nu_\eps(s),a)-\wtilde Q^\pi(s,a)\qquad\qquad \textit{ where } a=\argmax_{a_2}\wtilde Q^\pi(s,a_2)\\
&\geq     -L_s \cdot \eps
\end{align*}
The bound on the other side can be similarly derived.

Next, we compute the certified radius at state $s$. 
Let $\hat s$ be the adversarial state observation satisfying the constraint $\norm{\hat s-s}\leq \eps$. 
Leveraging the property that $\eta_s_a$ is $1$-\lip in $\cal N(s)$ given in~\Cref{lem:1-lip}, we have
% compute the certified radius as follows.
% For any $\delta$ with $\norm{\delta}_2\leq \eps$,
\begin{align}
    \label{eq:r-1}
    & \left(\textit{Due to \lip continuity}\right) 
    & \eta_{\hat s}^{(a_1)}(s) - \eta_{\hat s}^{(a_1)}(\hat s) \leq \eps \\
    \label{eq:r-2}
    & \left(\textit{Property of adversarial example}\right) 
    & \eta_{\hat s}^{(a_1)}(\hat s) \leq \eta_{\hat s}^{(a_2)}(\hat s)\\
    % \label{eq:r-3}
    % & \left((\textit{\ref{eq:r-1}) + (\ref{eq:r-2})}\right) 
    % & \eta_{a_1}(s) \leq \eta_{a_2} (\hat s) + \norm{\delta}_2\\
    \label{eq:r-4}
    & \left(\textit{Due to \lip continuity}\right)
    & \eta_{\hat s}^{(a_2)}(\hat s) - \eta_{\hat s}^{(a_2)}(s) \leq \eps\\
    \label{eq:r-5}
    & \left(\textit{(\ref{eq:r-1}) + (\ref{eq:r-2}) + (\ref{eq:r-4})}\right) 
    & \eta_{\hat s}^{(a_1)}(s) - \eta_{\hat s}^{(a_2)}(s) \leq 2\eps.
\end{align}
Thus, to allow for the existence of an adversarial example within perturbation budget $\eps$, the following condition needs to be satisfied:
\begin{align}
    \label{eq:r-cond}
    \eps 
    &\geq \min_{\substack{s'\\\st\norm{s'-s}_2\leq \eps}} \frac{1}{2}\left( \eta_{\hat s}^{(a_1)}(s) - \eta_{\hat s}^{(a_2)}(s) \right).
\end{align}
The certified radius $R(s)$ at state $s$ is thus the smallest $\eps$ for Ineq. (\ref{eq:r-cond}) to hold.


Thus, the magnitude of the perturbation applied to state $s$ shall at least 

in order to mislead the action given by $\tilde \pi$, the perturbation magnitude shall at least be 
% $\frac{1}{2}\left(\eta_{a_1}(s) - \eta_{a_2} (s)\right)$, \ie,
% which implies that the induced action will not change within
\begin{align*}
        R(s) &= \frac{1}{2}\left(\eta_{a_1}(s) - \eta_{a_2} (s)\right) \\
             &=
        \frac{\sigma}{2}\left(
    \Phi^{-1}\left(\frac{\wtilde Q(s,a_1)-V_{\min}}{V_{\max}-V_{\min}}\right)-
    \Phi^{-1}\left(\frac{\wtilde Q(s,a_2)-V_{\min}}{V_{\max}-V_{\min}}\right)
    \right).
\end{align*}
\end{proof}
\fi


==> archive/thm-q-bound.tex <==
\begin{theorem}
\label{thm:radius}
% Let $Q^\pi$ be the action value function given by the trained $Q$ network with policy $\pi$.
% Assume $\wtilde Q^\pi$ is the smoothed $Q^\pi$ given by~\Cref{eq:smooth-q}, and $\tilde\pi$ is the policy induced by the smoothed action value function $\wtilde Q^\pi$ following~\Cref{alg:smooth-q}.
Let $Q^\pi: \cal S \times \cal A\rightarrow \bb R$ be a trained value network, 
$\wtilde Q^\pi$ be the smoothed action-value function given in~\Cref{eq:smooth-q} and $\wtilde V^\pi$ be the smoothed value function given in~\Cref{eq:smooth-v}.
We further define $\wtilde V_\eps^\pi(s) := \wtilde V^\pi (s + \nu_\eps(s)) $ as the test-time value function given a perturbation $\nu_\eps(s):\cal S\rightarrow \cal S$ within magnitude $\eps$ on the input state observation $s$.
Then for any $s\in \cal S$,
\begin{align*}
    |\wtilde V_\eps^\pi(s)-\wtilde V^\pi(s)|\in [-L_s\eps, L_s\eps].
\end{align*}
Further, we can certify a radius $R$ at state $s$, such that when the perturbation scale is smaller than $R(s)$, the induced action at state $s$ will not change. The radius $R(s)$ is defined below
\begin{align*}
    R(s)
    &:= \frac{1}{2}\left( \eta_{a_1}(s) - \eta_{a_2}(s) \right).
\end{align*}
% \begin{align*}
%         R(s) := \frac{\sigma}{2}\left(
%     \Phi^{-1}\left(\frac{\wtilde Q(s,a_1)-V_{\min}}{V_{\max}-V_{\min}}\right)-
%     \Phi^{-1}\left(\frac{\wtilde Q(s,a_2)-V_{\min}}{V_{\max}-V_{\min}}\right)
%     \right),
% \end{align*}
where $a_1$ is the action of the highest smoothed $\wtilde Q$ value, while $a_2$ is the runner-up action.
\end{theorem}


==> certify-algs.tex <==
{


\section{Na\"ive Certification Approaches for Actual Reward Bounds}

    This section contains the certification approaches considering the actual reward bounds.
    These algorithms are suitable for both value-based neural networks and policy-based neural networks.
    
    \subsection{Notations}
        Given a \emph{deterministic} policy $\pi$, we define the \emph{actual reward} by
        \begin{align}
            \bar Q^\pi(s,a) & := \E\left[ \sum_{t=0}^\infty \gamma^t r_t \Big| s_0 = s, a_0=a, \pi\right], \\
            \bar V^\pi(s) & := \E\left[ \sum_{t=0}^\infty \gamma^t r_t \Big| s_0 = s, \pi\right], \\
            J(\pi) & := \E\left[\sum_{t=0}^\infty \gamma^t r_t \Big| s_0 \sim d_0, \pi\right].
        \end{align}

    \subsection{Certifying Globally Randomized Policy: Global Smoothing}
    
        For the given deterministic policy $\pi$, we construct a randomized policy $\pi'$.
        At each step, this randomized policy $\pi'$ adds one-time perturbation $\delta \sim \gN(0,\sigma^2I)$ to the observed state $s$, and make decision according to $\pi(s + \delta)$.
        Note that that $\pi'$ is different from the smoothed policy defined in main text.
        Because at each step, we just add one noise and make the decision according to this single noised state instead of adding multiple noises and make the decision according to the majority vote.
        
        We assume that each epoch has at most $H$ time steps, each state has $s$ dimensions.
        Then, we define a function $F: \sR^{H \times S} \to \sR$ such that
        \begin{align}
            F(\delta_1,\delta_2,\dots,\delta_H) = \E
            \left[
                \sum_{t=0}^H \gamma_t r_t \Big| s_0 \sim d_0, s_i = \pi(s_{i-1}, \delta_i)
            \right],
        \end{align}
        where $\delta_i \in \sR^S$ is the perturbation added to each step.
        Furthermore, we define smoothed $F$ by $\tilde F: \sR^{H\times S} \to \sR$:
        \begin{align}
            & \tilde F(s_1,s_2,\dots,s_H) \nonumber \\
            = & 
            \underset{\substack{\delta_i \sim \gN(0,\sigma^2I_S),\\ 1\le i\le H}}{\E} F(s_1+\delta_1,s_2+\delta_2,\dots,s_H+\delta_H).
        \end{align}
        
        According to the definition, 
        \begin{align}
            J(\pi') = \underset{\substack{\delta_i \sim \gN(0,\sigma^2I_S),\\ 1\le i\le H}}{\E} F(\delta_1,\delta_2,\dots,\delta_H) = \tilde F(0,\dots,0).
        \end{align}
        We let $(\delta_1',\delta_2',\cdots,\delta_H')$ be the state perturbation added to each step.
        Then, the resulting actual reward received under the perturbation by policy $\pi'$ is exactly
        \begin{align}
            \tilde F(\delta_1',\delta_2',\cdots,\delta_H').
        \end{align}
        As a result, we can sample to estimate $\tilde F(0,\cdots,0) = J(\pi')$~(using Hoeffding's Inequality to get a high confidence bound).
        Then, we can leverage the smoothness property of $\tilde F$~\cite{salman2019provably,chiang2020detection} to obtain a lower bound of $\tilde F(\delta_1', \delta_2', \dots,\delta_H')$, which is a valid certification of the actual reward for the randomized policy $\pi'$.

        \begin{remark}
            Regardless of the input dimension, the certification of the smoothed function has a similar magnitude as long as the noise variance $\sigma$ is the same.
            For example, when $\sigma = 1.0$, the non-trivial robustness certification usually requires the perturbation be bounded by $\ell_2$ under $1.0$---$2.0$.
            Thus, if the input dimension is too high, the permitted noise per component is too small~(scales down in $1/\sqrt{d}$ rate).
            
            For the classification, the input dimension is exactly the image size.
            However, for reinforcement learning, this global smoothing strategy produces an input dimension $H\times S$.
            If the state is an image, it is about $H$ times larger than the dimension of the classification task.
            Therefore, the certified robustness would be coarse.
            
            A potential direction is to reduce the dimension of state observation.
            We may train the policy in low-dimensional space, and certify the projection from high dimension to low dimension is robust. 
            Then the whole pipeline may have nontrivial certified robustness.
            The idea would be in spirit similar to low-rank approximation for certified robustness~\cite{awasthi2020adversarial}.
        \end{remark}
        
        \begin{remark}
            To yield a good randomized policy $\pi'$, the original policy should be trained to still have good performance under Gaussian corrupted state observations.
            In other words, it is necessary to train the policy using Gaussian augmentation on the state observation.
        \end{remark}
    
        % \fan{pseudo code see~\Cref{alg:global-rand}}
        % \input{pseudo-code/global-certify}
    
    \subsection{Certifying Stepwise Smoothed Policy: Adaptive Search}
        
        
        \paragraph{Prerequisite.}
        Either the test environment supports state saving or backtracking, either the state transition is deterministic.
        
        For the given deterministic policy $\pi$, suppose the policy uses per-step smoothing, which corresponding to using $\tilde Q$ for value network or pure smoothing for policy network.
        Then, at each step $i$, we can easily derive a certified robust radius $r_i$, such that the perdicted action $a_i$ does not change as long as the state observation is perturbed within $\ell_2$ radius $r_i$.
        Moreover, by comparing the smoothed confidence for each action, or the smoothed $\tilde Q$ for each action, we can know that if the perturbation goes beyond $r_i$, what action(s) it might take.
        Formally,
        we would have $r_{i,a'}$ for each action $a'$ different from the benign action, such that within $r_{i,a'}$ at least the policy would not choose $a'$.
    
        We assume that the initial state is fixed to $s_0$.
        
        First, we run the policy $\pi$ without any state perturbation starting from $s_0$, until it finishes an epoch with $H$ time steps.
        We record the actual reward as $J(\pi)$ and the per-step certified radius as $r_i$ where $1\le i\le H$.
        Now, we know the actual reward lower bound is $J(\pi)$ as long as the perturbation per step is within $\min_{1\le i\le H} r_i$.
        
        For notation simplicity, we let $i_0 = \argmin_{1\le i\le H} r_i$.
        Thus, $\min_{1\le i\le H} r_i = r_{i_0}$.
        
        We start to enlarge the radius from $r_{i_0}$.
        We spot the runner-up action at step $i_0$, which is denoted as $a^{adv}_{i_0}$.
        We then figure out $r^{new}$, such that under perturbation within $r^{new}$, for all steps other than $i_0$ it is still robust, and only on step $i_0$, we may choose either $a_{i_0}$ or $a^{adv}_{i_0}$.
        Apparently, we have $r^{new} > r_{i_0}$.
        We start to explore the trajectory $s_0,a_0,s_1,a_0,\cdots,s_{i_0},a_{i_0}^{adv}$.
        For the steps $i$'s following $i_0$, we explore all possible actions $a$ with certified radius $r_{i,a} \le r_{i_0}$.
        We record the lowest actual reward we get as $J'$.
        Then, the actual reward lower bound is $J'$ as long as the perturbation is within $r^{new}$.
        Here, $r^{new}$ is the minimum certified radius that is  larger than $\min_{1\le i\le H} r_i$ among all steps we encountered during the process.
        
        We repeat the process to enlarge the radius from $r^{new}$.
        The process can be viewed as generating new branches from a trajectory tree.
        The algorithm can be terminated at any time.
        As a possible optimization, notice the decay factor $\gamma$---we may do early stopping with bounded loss to accelerate.
        
        \begin{remark}
            At a high level, the algorithm is based on search.
            It goes through all possible trajectories to find the actual reward lower bound.
            The per-step smoothing provides the guarantee that we can determine all possible trajectories given the perturbation budget, which otherwise impossible.
        \end{remark}
        
        \begin{remark}
            In the supervised learning setting, for most samples, the certified radii are large.
            Only for a few samples, the certified radii are small.
            Simiarly, I conjecture that in the reinforcement learning case, there are just few steps with small certified radii.
            Thus, as long as we branch and search all these few steps, we can significantly enlarge the certified radius.
        \end{remark}
        
        \begin{remark}
            The existence of this algorithm also implies that, to certify the actual reward lower bound for a deterministic policy~(instead of expectation as before), maybe it is inevitable to examine every possible trajectory,
            since we do not know what would happen on the unexplored trajectory.
            It is essentially because we do not have the smoothness guarantee of $Q^*$, which is solely depended on the internal properties of the game and the reward. 
        \end{remark}
        
        % \fan{pseudo code see~\Cref{alg:adaptive-search}}
        % \input{pseudo-code/adaptive-search}
    
}

==> fig_desc/fig_Breakout_lore.tex <==
\renewcommand{\thesubfigure}{\alph{subfigure}}


\begin{figure}



\newlength{\utilheightbreakout}
\settoheight{\utilheightbreakout}{\includegraphics[width=.3\linewidth]{figures/Breakout_adasearch_sigma-0.005.pdf}}%


\newlength{\legendheightbreakout}
\setlength{\legendheightbreakout}{0.25\utilheightbreakout}%


\newcommand{\rowname}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightbreakout][c]{\small #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightbreakout]{figures/legend_Breakout.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}}
        & \makecell{\small{$\sigma=0.005$}}
        & \makecell{\small{$\sigma=0.01$}}
        & \makecell{\small{$\sigma=0.05$}}
        \vspace{-2pt}\\
\rowname{\makecell{(Local) $\uj$}}&
\includegraphics[height=\utilheightbreakout]{figures/Breakout_adasearch_sigma-0.005.pdf}&
\includegraphics[height=\utilheightbreakout]{figures/Breakout_adasearch_sigma-0.01.pdf}&
\includegraphics[height=\utilheightbreakout]{figures/Breakout_adasearch_sigma-0.05.pdf}
\\[-0.1ex]
        & \makecell{\small{attack epsilon $\eps$}}
        & \makecell{\small{attack epsilon $\eps$}}
        & \makecell{\small{attack epsilon $\eps$}}
\end{tabular}
% }
% \caption{\small Certified radius $R_t$ along time steps}\label{tab:cert-rad}
\end{subtable}

}
\vspace{-3mm}
\caption{\small \mo{\textbf{Robustness certification for cumulative reward lower bound $\uj$  on \textit{Breakout}}. We evaluate the trajectory length $H=200$. Each column corresponds to one smoothing parameter $\sigma$. Different lines represent the certified reward bounds of different RL methods.}
}%
\label{fig:breakout-lore}
\end{figure}



==> fig_desc/fig_global.tex <==
{
\renewcommand{\thesubfigure}{\alph{subfigure}}
% {\refstepcounter{subfigure}\textbf{(\thesubfigure) }{\ignorespaces #1}}

\begin{figure}



\newlength{\utilheightc}
\settoheight{\utilheightc}{\includegraphics[width=.155\linewidth]{figures/Freeway_global_mean_sigma-0.001.pdf}}%

\newlength{\utilheightd}
\settoheight{\utilheightd}{\includegraphics[width=.155\linewidth]{figures/Freeway_global_median_sigma-0.001.pdf}}%


\newlength{\utilheightaa}
\settoheight{\utilheightaa}{\includegraphics[width=.155\linewidth]{figures/Freeway_adasearch_sigma-0.001.pdf}}%

\newlength{\utilheightab}
\settoheight{\utilheightab}{\includegraphics[width=.155\linewidth]{figures/Pong_adasearch_sigma-0.001.pdf}}%

% \newlength{\utilheight}
% \settoheight{\utilheight}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: low degree.pdf}}%

% \newlength{\attackheightb}
% \settoheight{\attackheightb}{\includegraphics[width=.138\linewidth]{figures/twitch-DE: high degree.pdf}}%

\newlength{\legendheightb}
\setlength{\legendheightb}{0.3\utilheightc}%


\newcommand{\rownamec}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightc][c]{\footnotesize #1}}}

\newcommand{\rownamed}[1]% #1 = text
{\rotatebox{90}{\makebox[\utilheightd][c]{\footnotesize #1}}}

\centering



{
\renewcommand{\tabcolsep}{10pt}


\begin{subtable}[]{\linewidth}
\begin{tabular}{l}
\includegraphics[height=\legendheightb]{figures/legend.pdf}
\end{tabular}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
        & \makecell{\footnotesize{$\sigma=0.005$}}
        & \makecell{\footnotesize{$\sigma=0.05$}}
        & \makecell{\footnotesize{$\sigma=0.1$}}
        & \makecell{\footnotesize{$\sigma=0.5$}}
        & \makecell{\footnotesize{$\sigma=0.75$}}
        & \makecell{\footnotesize{$\sigma=1.0$}}
        \vspace{-1.7pt}\\
\rownamec{\makecell{Freeway}}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.005.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.01.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.05.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.1.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.5.pdf}&
\includegraphics[height=\utilheightc]{figures/Freeway_global_mean_sigma-0.75.pdf}\\[-1.2ex]
\rownamec{\makecell{Pong}}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.001.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.005.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.01.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.05.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.1.pdf}&
\includegraphics[height=\utilheightc]{figures/Pong_global_mean_sigma-0.1.pdf}\\[-1.2ex]
\end{tabular}
% }
\caption{\small Expectation bound $\uje$: lower bound of $\ujefull$ w.r.t. $\eps$}\label{tab:ebound}
\end{subtable}

\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\rownamed{\makecell{Freeway}}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.005.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.01.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.05.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.1.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.5.pdf}&
\includegraphics[height=\utilheightd]{figures/Freeway_global_median_sigma-0.75.pdf}\\[-1.2ex]
\rownamed{\makecell{Pong}}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.001.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.005.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.01.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.05.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.1.pdf}&
\includegraphics[height=\utilheightd]{figures/Pong_global_median_sigma-0.1.pdf}\\[-1.2ex]
\end{tabular}
% }
\caption{\small Percentile bound $\ujp$: lower bound of the $p$-th percentile of $\jfull$ w.r.t. $\eps$, with $p=50\%$}\label{tab:pbound}
\end{subtable}


\begin{subtable}[]{\linewidth}
\centering
% \resizebox{\linewidth}{!}{%
\begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\rownamed{\makecell{Freeway}}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.005.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.05.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.1.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.5.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-0.75.pdf}&
\includegraphics[height=\utilheightaa]{figures/Freeway_adasearch_sigma-1.0.pdf}\\[-1.2ex]
\rownamed{\makecell{Pong}}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.001.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.005.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.01.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.03.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.05.pdf}&
\includegraphics[height=\utilheightab]{figures/Pong_adasearch_sigma-0.1.pdf}\\[-1.2ex]
\end{tabular}
% }
\caption{\small Absolute lower bound $\uj$: lower bound of $\jfull$ w.r.t. $\eps$, with a given initial state}\label{tab:abound}
\end{subtable}

% \begin{subtable}[]{\linewidth}
% \centering
% % \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}p{5mm}@{}c@{}c@{}c@{}c@{}c@{}c@{}}
% \rowname{\makecell{Freeway}}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.005.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.01.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.05.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.1.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.5.pdf}&
% \includegraphics[height=\utilheightd]{figures/Freeway_global_median_ratio_sigma-0.75.pdf}\\[-1.2ex]
% \rowname{\makecell{Pong}}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.001.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.005.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.01.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.05.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.1.pdf}&
% \includegraphics[height=\utilheightd]{figures/Pong_global_median_ratio_sigma-0.5.pdf}\\[-1.2ex]
% \end{tabular}
% % }
% \caption{\small Certified ratio}\label{tab:cert-ratio}
% \end{subtable}
}
\caption{\small Certification for cumulative reward, including (a) expectation bound, (b) percentile bound, and (c) absolute lower bound for different models. Each column corresponds to one smoothing variance and each colored curve shows the result of one method as depicted in the legend.
\fan{Figures incomplete.}
}%
\label{fig:global-bound}
\end{figure}

}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> pseudo-code/adaptive-search-skipframe.tex <==
\begin{algorithm}[t]
\algsetup{linenosize=\tiny}
\scriptsize
\DontPrintSemicolon
\KwIn{initial state distribution $d_0$, deterministic transition function $\Gamma(s,a)$, deterministic immediate reward function $r(s,a)$; trained value network $Q^\pi$; parameters for randomized smoothing: sampling times $m$, smoothing variance $\sigma^2$, one-sided confidence level parameter $\alpha$; frame skipping gap $k$}
\KwOut{a map $certify\_map$ that maps a radius $rad$ to the corresponding certified lower bound of reward $re$}
\SetKwFunction{funca}{get\_actions}
\SetKwFunction{funcb}{expand}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\Comment*[l]{\footnotesize Initialize global variables}
$p\_que \leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize an empty priority queue containing tuples of (state $s$, action $a$, radius $rad$, reward $re$) (sorted by increasing $rad$)}
$certify\_map \leftarrow \emptyset$\; % \Comment*[r]{\scriptsize initialize an empty map that maps a radius $rad$ to the certified lower bound of reward $re$}
$re\_min \leftarrow \infty$ \Comment*[r]{\scriptsize initialize global minimum reward}
$state\_set\leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize a set for visited states}
$state\_dict\leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize a map for visited states at current radius}
Generate noise samples $\delta_j\sim \cal N(0, \sigma^2I)$ for $1\leq j\leq m$\; 
$V_{\min}, V_{\max}\leftarrow$ sampled minimum and maximum value of the given network $Q^\pi$\;
$\Delta =  \left( V_{\max} - V_{\min}\right) \sqrt{\frac{1}{2m} \ln \frac{1}{\alpha}}$ \Comment*[r]{\scriptsize Hoeffding's bound under $\alpha$ confidence level}\;

\Fn{\funca{$s,a\_seq, rad\_lim, re\_cur$}}{
    $vis\leftarrow $ \texttt{False}\;
    \If { $s$ in $state\_set$ } {
        $vis\leftarrow $ \texttt{True}\;
    }
    $state\_set.\texttt{add}(s)$\;
    $k_s \leftarrow \texttt{len}(a\_seq)$\;
    $re\_accum \leftarrow 0$\;

    \For {$i$ from $1$ to $k_s-1$} { \Comment*[r]{\scriptsize skipping the first $k_s-1$ frames}
        $a \leftarrow a\_seq[i]$\;
        $re\_accum \leftarrow re\_accum + r(s, a)$\;
        $s \leftarrow \Gamma(s, a)$\;
        \If {$s = \bot$} {
            \KwRet $\bot, re\_accum$\;
        }
    }
    $a\_last \leftarrow a\_seq[k_s]$ \;
    $\wtilde Q^\pi(s,a) \leftarrow \frac{1}{m} \sum_{j=1}^{m}\texttt{clip}\left( Q^\pi(s+\delta_j, a), \min=V_{\min}, \max=V_{\max}\right)$\;
    $a^\star\leftarrow \argmax_{a\in\cal A} \wtilde Q^\pi(s,a)$\;
    % $re\leftarrow re\_cur + r(s,a)$\;
    \uIf {$\wtilde Q^\pi(s,a^\star) \geq \wtilde Q^\pi(s,a\_last)+2\Delta$} {
        $rad\leftarrow \frac{\sigma}{2}\left(
                                            \Phi^{-1}\left(\frac{\wtilde Q^\pi(s,a^\star)-\Delta-V_{\min}}{V_{\max}-V_{\min}}\right)-
                                            \Phi^{-1}\left(\frac{\wtilde Q^\pi(s,a)+\Delta-V_{\min}}{V_{\max}-V_{\min}}\right)
                                        \right)$\;
    }
    \Else {
        $rad \leftarrow $ 0\;
    }
    
    \uIf{$rad\leq rad\_lim$} {
        $re\_accum \leftarrow re\_accum + r(s, a\_last)$\;
        \KwRet $\Gamma(s, a\_last), re\_accum$ \Comment*[r]{\scriptsize take the possible action within $rad\_lim$}
    }
    \uElseIf {not $vis$} {
        $p\_que.\texttt{push}((s, a\_last, rad, re\_cur + re\_accum))$ \Comment*[r]{\scriptsize put currently impossible actions in queue}
        \KwRet $\texttt{Null}, re\_accum$\;
    }
}
\;
\Pn{\funcb{$s,rad\_lim, re\_cur$}}{
    \If {$re\_cur \geq re\_min$} {
        \KwRet{$0$} \Comment*[r]{\scriptsize pruning}
    }
    $k_s \leftarrow \min(k, estimated\_hit\_gap)$\;
    \Comment*[r]{\scriptsize estimate the time gap till the next frame where the ball hits the paddle}
    $a\_seq\_list \leftarrow \{[0,0,\ldots,0],
                                \underbrace{[1,0,\ldots,0],[1,1,\ldots,0],\ldots, [1,1,\ldots,1]}_{k_s \text{ sequences}},
                                \underbrace{[-1,0,\ldots,0],[-1,-1,\ldots,0],\ldots, [-1,-1,\ldots,-1]}_{k_s \text{ sequences}}\}$\;
    \Comment*[r]{\scriptsize $2k_s+1$ action sequences, where $\{-1,0,1\}$ means moving up / moving down / staying still}
    \For {$a\_seq \in a\_seq\_list$} {
        $s', re\_accum \leftarrow \funca{s, a\_seq, rad\_lim, re\_cur}$\;
        \uIf {$s' = \bot$} {
            $re\_min \leftarrow \min (re\_min, re\_cur + re\_accum)$\;
        }
        \uElseIf {$ s' \neq \texttt{Null}$} {
            \uIf {$s'$ in $state\_dict$} {
                $re\_ftr \leftarrow \min(re\_ftr, state\_dict[s'] + re\_accum)$\;
                $re\_min \leftarrow \min(re\_min, re\_cur + re\_accum)$\;
                % \textbf{continue}\;
            }
            \Else {
                $ret \leftarrow \funcb{s', rad\_lim, re\_cur + re\_accum} $\;
                $state\_dict[s'] \leftarrow \min(state\_dict[s'], ret)$\;
                $re\_ftr \leftarrow \min(re\_ftr, ret + re\_accum)$
            }
        }
    }
    \KwRet $re\_ftr$\;    
    % $a\_list \leftarrow \funca(s,rad\_lim, re\_cur)$\;
    % \If {$a\_list = \emptyset$} {
    %     $re\_min \leftarrow \texttt{min}(re\_min, re\_cur)$\;
    %     \KwRet{$0$}\;
    % }
    % $re\_ftr\leftarrow \infty$\;
    % \For {$a \in a\_list$} {
    %     $s'\leftarrow \Gamma(s,a)$\;
    %     \If { $s'$ in $state\_dict$ } {
    %         $re\_ftr\leftarrow\min(re\_ftr, state\_dict[s']+r(s,a))$\;
    %         $re\_min\leftarrow \min(re\_min, re\_cur+r(s,a))$\;
    %         \textbf{continue} \Comment*[r]{\scriptsize skip visited states}
    %     }
    %     $ret\leftarrow \funcb(s',rad\_lim, re\_cur+r(s,a))$\;
    %     $state\_dict[s'] = \min(state\_dict[s'], ret)$\;
    %     $re\_ftr\leftarrow \min(re\_ftr, ret+r(s,a))$\;
    % }
    % \KwRet{$re\_ftr$}\;
}
\;
$s_0\sim d_0$ \Comment*[r]{\scriptsize initialize initial state}
\funcb($s_0, rad\_lim=0,re\_cur=0$) \Comment*[r]{\scriptsize expand initial trajectory}
\While {True} {
    \If {$p\_que = \emptyset$} {
        \textbf{break}\;
    }
    $(s,a,rad,re)\leftarrow p\_que.\texttt{pop}()$ \Comment*[r]{\scriptsize pop out the first element of the priority queue}
    $state\_dict\leftarrow \emptyset$\;
    $certify\_map[rad] \leftarrow re\_min$ \Comment*[r]{\scriptsize the certified lower bound of reward at $rad$ is $re\_min$}
    $(s',a',rad',re')\leftarrow p\_que.\texttt{top}()$ \Comment*[r]{\scriptsize examine the first element of the updated priority queue}
    \funcb$(\Gamma(s,a), rad', re+r(s,a))$ \Comment*[r]{\scriptsize expand the tree from the new state}
}
\caption{Adaptive Search with Frame Skipping}\label{alg:adaptive-search}
\end{algorithm}



==> pseudo-code/adaptive-search.tex <==
\begin{algorithm}[!ht]
\algsetup{linenosize=\tiny}
\scriptsize
\DontPrintSemicolon
\KwIn{initial state distribution $d_0$, deterministic transition function $\Gamma(s,a)$, deterministic immediate reward function $r(s,a)$; trained value network $Q^\pi$; parameters for randomized smoothing: sampling times $m$, smoothing variance $\sigma^2$, one-sided confidence level parameter $\alpha$}
\KwOut{a map $certify\_map$ that maps a radius $rad$ to the corresponding certified lower bound of reward $re$}
\SetKwFunction{funca}{\textsc{GetAction}}
\SetKwFunction{funcb}{\textsc{Expand}}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\Comment*[l]{\footnotesize Initialize global variables}
$p\_que \leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize an empty priority queue containing tuples of (state $s$, action $a$, radius $rad$, reward $re$) (sorted by increasing $rad$)}
$certify\_map \leftarrow \emptyset$\; % \Comment*[r]{\scriptsize initialize an empty map that maps a radius $rad$ to the certified lower bound of reward $re$}
$re\_min \leftarrow \infty$ \Comment*[r]{\scriptsize initialize global minimum reward}
$state\_set\leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize a set for visited states}
$state\_dict\leftarrow \emptyset$ \Comment*[r]{\scriptsize initialize a map for visited states at current radius}

$V_{\min}, V_{\max}\leftarrow$ sampled minimum and maximum value of the given network $Q^\pi$\;
$\Delta =  \left( V_{\max} - V_{\min}\right) \sqrt{\frac{1}{2m} \ln \frac{1}{\alpha}}$ \Comment*[r]{\scriptsize Hoeffding's bound under $\alpha$ confidence level}\;

\Fn{\funca{$s,rad\_lim, re\_cur$}}{
    $vis\leftarrow $ \texttt{False}\;
    \If { $s$ in $state\_set$ } {
        $vis\leftarrow $ \texttt{True}\;
    }
    $state\_set.\texttt{add}(s)$\;
    Generate noise samples $\delta_i\sim \cal N(0, \sigma^2I)$ for $1\leq i\leq m$\; 
    \For {each action $a\in \cal A$} {
        $\wtilde Q^\pi(s,a)\leftarrow \frac{1}{m} \sum_{i=1}^{m}\texttt{clip}\left( Q^\pi(s+\delta_i, a), \min=V_{\min}, \max=V_{\max}\right)$\;
    }
    $a^\star\leftarrow \argmax_{a\in\cal A} \wtilde Q^\pi(s,a)$\;
    $a\_list\leftarrow \emptyset$\;
    \For {each action $a\in \cal A$} {
        \If {$\Gamma(s,a)=\bot$} {
            \textbf{continue}\;
        }
        % $re\leftarrow re\_cur + r(s,a)$\;
        \uIf {$\wtilde Q^\pi(s,a^\star) \geq \wtilde Q^\pi(s,a)+2\Delta$} {
            $rad\leftarrow \frac{\sigma}{2}\left(
                                                \Phi^{-1}\left(\frac{\wtilde Q^\pi(s,a^\star)-\Delta-V_{\min}}{V_{\max}-V_{\min}}\right)-
                                                \Phi^{-1}\left(\frac{\wtilde Q^\pi(s,a)+\Delta-V_{\min}}{V_{\max}-V_{\min}}\right)
                                            \right)$\;
        }
        \Else {
            $rad \leftarrow $ 0\;
        }
        
        \uIf{$rad\leq rad\_lim$} {
            $a\_list\leftarrow a\_list \cup \{a\}$ \Comment*[r]{\scriptsize take the possible action within $rad\_lim$}
        }
        \uElseIf {not $vis$} {
            $p\_que.\texttt{push}((s, a, rad, re\_cur))$ \Comment*[r]{\scriptsize put currently impossible actions in queue for later expansion}
        }
    }
    \KwRet{$a\_list$}\;
}
\;
\Pn{\funcb{$s,rad\_lim, re\_cur$}}{
    \If {$re\_cur \geq re\_min$} {
        \KwRet{$0$} \Comment*[r]{\scriptsize pruning}
    }
    $a\_list \leftarrow \funca(s,rad\_lim, re\_cur)$\;
    \If {$a\_list = \emptyset$} {
        $re\_min \leftarrow \texttt{min}(re\_min, re\_cur)$\;
        \KwRet{$0$}\;
    }
    $re\_ftr\leftarrow \infty$\;
    \For {$a \in a\_list$} {
        $s'\leftarrow \Gamma(s,a)$\;
        \If { $s'$ in $state\_dict$ } {
            $re\_ftr\leftarrow\min(re\_ftr, state\_dict[s']+r(s,a))$\;
            $re\_min\leftarrow \min(re\_min, re\_cur+r(s,a))$\;
            \textbf{continue} \Comment*[r]{\scriptsize skip visited states}
        }
        $ret\leftarrow \funcb(s',rad\_lim, re\_cur+r(s,a))$\;
        $state\_dict[s'] = \min(state\_dict[s'], ret)$\;
        $re\_ftr\leftarrow \min(re\_ftr, ret+r(s,a))$\;
    }
    \KwRet{$re\_ftr$}\;
}
\;
$s_0\sim d_0$ \Comment*[r]{\scriptsize initialize initial state}
\funcb($s_0, rad\_lim=0,re\_cur=0$) \Comment*[r]{\scriptsize expand initial trajectory}
\While {True} {
    \If {$p\_que = \emptyset$} {
        \textbf{break}\;
    }
    $(s,a,rad,re)\leftarrow p\_que.\texttt{pop}()$ \Comment*[r]{\scriptsize pop out the first element of the priority queue}
    $state\_dict\leftarrow \emptyset$\;
    $certify\_map[rad] \leftarrow re\_min$ \Comment*[r]{\scriptsize the certified lower bound of reward at $rad$ is $re\_min$}
    $(s',a',rad',re')\leftarrow p\_que.\texttt{top}()$ \Comment*[r]{\scriptsize examine the first element of the updated priority queue}
    \funcb$(\Gamma(s,a), rad', re+r(s,a))$ \Comment*[r]{\scriptsize expand the tree from the new state}
}
\caption{\adasearch: Adaptive Search}\label{alg:adaptive-search-full}
\end{algorithm}



==> pseudo-code/gaussian-aug.tex <==
\begin{algorithm}[t]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
% \KwOut{action $a$}
\DontPrintSemicolon
Initialize replay buffer $D=\emptyset$\;
Initialize action-value function $Q$ with random weight $\theta$\;
Initialize target action-value function with weight $\theta^-=\theta$\;
\For {$episode=1$ to $M$}{
    Initialize state $s_1$\;
    % {\color{red}
    % \For {$t=1$ to $T$} {
    %     \For {$i=1$ to $n$} {
    %         $\eps_{ti}\leftarrow\cal N(0,\sigma^2)$\Comment*[r]{\scriptsize generate all perturbations beforehand}
    %     }
    % }
    % }
    \For {$t=1$ to $T$}{
        Following $\eps$-greedy policy, select $a_t=\arg\max_a Q(s_t,a;\theta)$ \wp $\eps$, or a random action otherwise\;
        Execute action $a_t$ and observe reward $r_t$ and next state $s_{t+1}$\;
        % {\color{red}
        % \For {$i=1$ to $n$}{
        %     \For {$j=1$ to $n$}{
        %         $\tilde s_t\leftarrow s_t+\eps_{t,i}$\;
        %         $\tilde s_{t+1}\leftarrow s_{t+1}+\eps_{t+1,j}$\;
        %         Store $(\tilde s_t,a_t,r_t,\tilde s_{t+1})$ in $D$ \Comment*[r]{\scriptsize store the smoothed transitions}
        %     }
        % }
        % }
        Sample random minibatch of transitions $(s_j,a_j,r_j,s_{j+1})$ from $D$ \Comment*[r]{\scriptsize Experience Replay}
        {\color{red}
        \Comment*[l]{\scriptsize Gaussian Data Augmentation}
        $\delta\leftarrow \cal N(0,\sigma^2)$ \;
        $\tilde s_j = s_j + \delta $\;
        $\tilde s_{j+1} = s_{j+1} + \delta $\;
        }
        $y_j\leftarrow r_j+\gamma \max_{a'}Q(\tilde s_{j+1},a';\theta^-)$\;
        Perform a gradient descent step on $(y_j-Q(\tilde s_j,a_j;\theta))^2$ \wrt the network parameter $\theta$\;
        Every $C$ steps set $\theta^-=\theta$ \Comment*[r]{\scriptsize Update the target network periodically}
    }
}
\caption{\textbf{[DQN]} Gaussian data augmentation during training}\label{alg:gaussian-augment}
\end{algorithm}


==> pseudo-code/local-certify.tex <==
\begin{algorithm}[t]
\algsetup{linenosize=\tiny}
  \footnotesize
% \KwIn{Q action-value function $Q$ with network parameter $\theta$, current state $s$, noise scale $\sigma$; parameter: nubmer of samples $n$}
\KwIn{state $s$, trained value network $Q^\pi$, one-sided confidence bound $\alpha$}
\KwOut{smoothed value network $\wtilde Q^\pi$, selected action $a$, certification flag $cert$, certified radius $R$, local \lip constant $L_s$; parameters for randomized smoothing: sampling times $m$, smoothing variance $\sigma^2$}
% \KwOut{action $a$}
\DontPrintSemicolon
\SetKwFunction{funcpgd}{projected\_gradient\_descent}
\SetKwFunction{funca}{compute\_cert\_R}
\SetKwFunction{funcb}{satisfy}
\SetKwProg{Pn}{Procedure}{:}{}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\funcpgd{$s,\eps$}} {
    objective function 
    \begin{align*}
        J=\min_{\substack{s'\\\st\norm{s'-s}_2\leq \eps}}
                \Phi^{-1}\left(\frac{\widetilde{Q}\left(s, a_1\right)-\Delta-l_{\mathcal{N}(s')}}{u_{\mathcal{N}(s')}-l_{\mathcal{N}(s')}}\right)
                    -
                \Phi^{-1}\left(\frac{\widetilde{Q}\left(s, a_2\right)+\Delta-l_{\mathcal{N}(s')}}{u_{\mathcal{N}(s')}-l_{\mathcal{N}(s')}}\right),
    \end{align*}
    where $\Delta=\left(u_{\mathcal{N}(s')}-l_{\mathcal{N}(s')}\right)\sqrt{\frac{1}{2m} \ln \frac{1}{\alpha}}$\;
    \KwRet{J}
}\;

\Fn{\funca{$s,\eps$}} {
    $J = \texttt{projected\_gradient\_descent}(s, \eps)$\;
    \If {$J = -1$} {
        \KwRet{$-1$}
    }
    $cert\_R \leftarrow \frac{\sigma}{2}J$\;
    \KwRet{$cert\_R$}\;
}\;

\Fn{\funcb{$cert\_R, \eps$}} {
    \KwRet{$\eps \geq cert\_R$}\;
}\;

\Comment*[l]{\footnotesize Main loop: binary search for the smallest R that satisfies ineq. (\ref{eq:r-cond})}
$hi\leftarrow 1, low\leftarrow 10^{-7}$\;
\While {$hi-low\geq 10^{-6}$} {
    $mid = (hi + low) / 2$\;
    $cert\_R \leftarrow \texttt{compute\_cert\_R}(s, \eps=mid)$\;
    \uIf {$cert\_R == -1$ or $\texttt{satisfy}(cert\_R, mid)$} {
        $hi \leftarrow mid$\;
    }
    \Else {
        $low \leftarrow mid$\;
    }
}
$R\leftarrow mid$\;
\KwRet $\wtilde Q$, $a_1$, $cert$, $R$, $L_s$\;
\caption{\small 
local \lip based randomized smoothing on action value function, along with the certification at given state.
}\label{alg:local-smooth-q}
\end{algorithm}


==> tables/tab_Breakout_lore.tex <==
{
\setlength{\tabcolsep}{4pt} % column sep

\begin{table}[]
    \centering

    \caption{\small \mo{\textbf{Empirical cumulative reward obtained under attacks of different magnitudes.}
    We follow~\citet{zhang2021robust} and~\citet{oikarinen2020robust} to conduct PGD attacks.
    We evaluate the trajectory length $H=200$. Each column group corresponds to one smoothing parameter $\sigma$. 
    For each smoothing parameter $\sigma$, we evaluate four attack magnitudes $\eps$.
    Different rows show the achieved empirical cumulative reward of different methods.}
    }
    \label{tab:breakout-lore}



\resizebox{\linewidth}{!}{%
        \begin{tabular}{c cccc cccc cccc
}
    \toprule
    \bm{$\sigma$} &  \multicolumn{4}{c}{$0.005$}  &  \multicolumn{4}{c}{$0.01$} &  \multicolumn{4}{c}{$0.05$}\\
    \cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
    % & \multicolumn{4}{c}{$\eps$}  &  \multicolumn{4}{c}{$\eps$} &  \multicolumn{4}{c}{$\eps$}\\ 
    \bm{$\eps$} &    \multicolumn{1}{c}{\small $5e-3$}  & \multicolumn{1}{c}{\makecell{\small $1e-2$}} & \multicolumn{1}{c}{\makecell{\small $5e-2$}} &  \multicolumn{1}{c}{\small $1e-1$} 
    &    \multicolumn{1}{c}{\small $5e-3$}  & \multicolumn{1}{c}{\makecell{\small $1e-2$}} & \multicolumn{1}{c}{\makecell{\small $5e-2$}} &  \multicolumn{1}{c}{\small $1e-1$}
    &    \multicolumn{1}{c}{\small $5e-3$}  & \multicolumn{1}{c}{\makecell{\small $1e-2$}} & \multicolumn{1}{c}{\makecell{\small $5e-2$}} &  \multicolumn{1}{c}{\small $1e-1$}
    \\\midrule
\textbf{ StdTrain } & 6 & 1 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 \\
\textbf{ GaussAug } & 6 & 5 & 5 & 1 & 6 & 5 & 5 & 1 & 0 & 0 & 0 & 0 \\
\textbf{ AdvTrain } & 6 & 6 & 0 & 0 & 7 & 7 & 0 & 0 & 0 & 0 & 0 & 0 \\
\textbf{ RegPGD } & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\
\bottomrule \\
\end{tabular}
}

\vspace{-5mm}
\end{table}
}

==> tx_draft.tex <==
\section{Performance Guarantees}

This section provides results on certificated robustness against perturbation on observation. 

Notations:
\begin{itemize}
\item Original value function (class): $f(\cdot,\cdot) \in \Fcal$
\item Smoothed function class: $\ftilde \coloneqq f(s,a) \circ \Ncal(0,\sigma^2 I) = \E_{\varepsilon \sim \Ncal(0,\sigma I)} \left[ f(s + \varepsilon, a)\right]$. $\widetilde \Fcal \coloneqq \{f \circ \Ncal(0,\sigma^2 I); f \in \Fcal\}$.
\item $f_1(s) = \max_{a \in \Acal} f(s,a)$
\item $f_2(s) = \max_{a \in \Acal \setminus a_s} f(s,a)$, where $a_s = \argmax_{a \in \Acal} f(s,a)$
\end{itemize}





\paragraph{Value-Based Approaches}

We now provide guarantees for the following procedure:
\begin{enumerate}
\item Approximate $Q^\star$ by $\Qhat$ in a unperturbed environment.
\item Smooth $\Qhat$ by $\Qtilde \coloneqq \Qhat \circ \Ncal(0,\sigma^2 I)$.
\item Output the greedy policy of $\Qtilde$.
\end{enumerate}

\begin{lemma}
\label{lem:tildelips}
$\Qtilde$ is $\frac{V_{\max}}{\sigma}\sqrt{\nicefrac{2}{\pi}}$-Lipschitz.
\end{lemma}

\begin{theorem}
Let $f$ be an arbitrary $L$-Lipschitz function, $\pi_{f}$ be the greedy policy of $f$, $\nu_\varepsilon$ denote arbitrary $L^2$ bounded observation perturbation. Then
\begin{align*}
J(\pi_{f}) - J(\pi_{f} \circ \nu_\varepsilon) \leq
\end{align*}
\end{theorem}

\begin{proof}
We now consider $Q^{\pi_{f}}$ and $Q^{\pi_{f} \circ \nu_\varepsilon}$.

\begin{align*}
&~ Q^{\pi_{f}}(s,\pi_f) - Q^{\pi_{f}}(s,\pi_{f} \circ \nu_\varepsilon)
\\
\leq &~ Q^{\pi_{f}}(s,\pi_f) - Q^{\pi_{f}}(s + \nu_\varepsilon(s),\pi_{f} \circ \nu_\varepsilon) + L_Q \varepsilon   \\ \tag{$Q^{\pi_{f}}$ is $L_Q$-Lipschitz by the MDP assumption}
\\
\leq &~ Q^{\pi_{f}}(s,\pi_f) - Q^{\pi_{f}}(s + \nu_\varepsilon(s),\pi_{f} \circ \nu_\varepsilon) + L_Q \varepsilon
\end{align*}

% \tx{It is not sure if only using $L$-Lipschitz $f$ is a sufficient condition to guarantee certificated robustness. If we also have $f$ closed to $Q^{\pi_f}$ (which is roughly $f \approx Q^\star$), then we are good. But things without that may not be doable.}

% \tx{For example, consider an extreme case --- $f$ is a constant function. In this case, $\pi_f$ and $\pi_{f} \circ \nu_\varepsilon$ can be two totally different policies.}

\end{proof}

